Analyzing and Improving the Optimization Landscape of Noise-Contrastive Estimation

Noise-contrastive estimation (NCE) is a statistically consistent method for learning unnormalized probabilistic models. It has been empirically observed that the choice of the noise distribution is crucial for NCE's performance. However, such observations have never been made formal or quantitative. In fact, it is not even clear whether the difficulties arising from a poorly chosen noise distribution are statistical or algorithmic in nature. In this work, we formally pinpoint reasons for NCE's poor performance when an inappropriate noise distribution is used. Namely, we prove these challenges arise due to an ill-behaved (more precisely, flat) loss landscape. To address this, we introduce a variant of NCE called "eNCE" which uses an exponential loss and for which normalized gradient descent addresses the landscape issues provably when the target and noise distributions are in a given exponential family.

==> draft_fix_proof_2d/calc_details/pos_b_neg_x.tex <==
The second term (i.e. $x < 0$) is very similar to the first term:
\begin{equation}
\begin{split}
    -&\int_{x<0} \frac{p}{\frac{p}{q}+1} x - \int_{x<0} \frac{p_*}{\frac{p}{q}+1} x
    \\
    =& -\frac{1}{\sqrt{2\pi}} \int_{x<0} \exp\left(-\frac{x^2}{2}\right)x
    - \frac{1}{\sqrt{2\pi}}\int_{x<0} \exp\left(-\frac{x^2}{2} + (R-b)x + c -\frac{R^2}{2} - \log\sqrt{2\pi}\right) x
    \\
    =& \frac{1}{\sqrt{2\pi}} \int_{x>0} \exp\left(-\frac{x^2}{2}\right)x
        + \frac{1}{\sqrt{2\pi}}\int_{x>0} \exp\left(-\frac{x^2}{2} - (R-b)x + c -\frac{R^2}{2} - \log\sqrt{2\pi}\right) x
    \\
    \overset{(i)}{=}& \begin{cases}
        1 + \frac{1}{(b-R)^2+1} \exp\left(-\frac{R^2}{2} + c - \log\sqrt{2\pi}\right),
        & R-b > 0
        \\
        1 + (R-b)\exp\left(\frac{b^2}{2} - Rb + c-\log\sqrt{2\pi}\right)
        + \frac{1}{(b-R)^2+1} \exp\left(-\frac{R^2}{2} + c - \log\sqrt{2\pi}\right),
        & R-b < 0
    \end{cases}
    \\
    =&\ O(1)
\end{split}
\end{equation}
Step $(i)$ omits a factor of $\frac{1}{\sqrt{2\pi}}$ and uses:
\begin{equation}
\begin{split}
    &\int_{x>0} \exp\left(-\frac{x^2}{2} - (R-b)x + c -\frac{R^2}{2} -2\log\sqrt{2\pi}\right) x
    \\
    =& \exp\left(\frac{(R-b)^2}{2} - \frac{R^2}{2} + c - \log\sqrt{2\pi}\right) \int_{x>0} \exp\left(-\frac{(x+(R-b))^2}{2}\right) x
    \\
    =& \exp\left(\frac{(R-b)^2}{2} - \frac{R^2}{2} + c - \log\sqrt{2\pi}\right) \left[ \int_{x>R-b} \exp\left(-\frac{x^2}{2}\right) x
        - (R-b) \int_{x>R-b}\exp\left(-\frac{x^2}{2}\right) \right]
    \\
    % =& \exp\left(-\frac{R^2}{2} + c -\log\sqrt{2\pi}\right)
    %     + T
    % \\
    \simeq& \begin{cases}
        \frac{1}{(b-R)^2+1} \exp\left(-\frac{R^2}{2} + c - \log\sqrt{2\pi}\right), & R-b > 0
        \\
        (R-b)\exp\left(\frac{b^2}{2} - Rb + c-\log\sqrt{2\pi}\right)
        + \frac{1}{(b-R)^2+1} \exp\left(-\frac{R^2}{2} + c - \log\sqrt{2\pi}\right)
        & R - b < 0
    \end{cases}
\end{split}
\end{equation}

==> proofs/claim_3rd_dev.tex <==
\subsection{[\textcolor{orange}{\textbf{not finished}}] Proof of Assumption \ref{assump:loss} (\texorpdfstring{$\|\nabla_{\param_*}^3 L\|_{\max}$}{max norm of the third order derivative}) on the NCE loss}

The second (i.e. Hessian) and third order derivative of the NCE loss at optimum are:
\begin{equation}
\begin{split}
    \nabla_{\param_*}^2 L
    =& \frac{1}{2} \int_x q(p_*+q)\cdot \frac{p}{(p+q)^2} T(x)^{\otimes 2} dx
    = \frac{1}{2}\int_x \frac{p_*q}{p_*+q} T(x)^{\otimes 2} dx
    \\
    \nabla_{\param_*}^3 L
    =& \frac{1}{2} \int_x q(p_*+q)\cdot \frac{p(q-p)}{(p+q)^3} \cdot T(x)^{\otimes 3} dx
    = \frac{1}{2}\int_x \frac{p_*q}{p_*+q} \cdot \frac{q-p_*}{p_*+q} \cdot T(x)^{\otimes 3} dx
    \\
\end{split}
\end{equation}
Since $\left|\frac{q-p_*}{p_*+q}\right| \leq 1$,
\footnote{This is likely quite tight, since e.g. when $\frac{q}{p_*} \gg 1$, $\frac{q - p_*}{p_* + q} \approx \frac{q}{q} = 1$;
the same goes for $\frac{q}{p_*} \ll 1$.}
we have
\begin{equation}
\begin{split}
    % \|\nabla_{\param_*}^3 L\|_{\max}
    % \leq \frac{1}{2}\left\|\int_{x} \frac{p_*q}{p_*+q} T(x)^{\otimes 3} dx\right\|_{\max}
    &2\nabla_{\param_*}^3 L (\vv, \vv, \vv)
    = \int_x \frac{p_*q}{p_*+q} \frac{q-p_*}{p_*+q} (\vv^\top T(x))^3
    \\
    \leq& \int_x \frac{pq}{p+q} \cdot \frac{q}{p+q} |\vv^\top T(x)|^3
        + \int_x \frac{pq}{p+q} \cdot \frac{p}{p+q} |\vv^\top T(x)|^3
    \\
    \overset{(*)}{\leq}& 2 \TxBdd \kappa_* \sigma_{\min}^*
\end{split}
\end{equation}
Step $(*)$ uses the following:
\begin{equation}
\begin{split}
    &\int_x \frac{pq}{p+q} \cdot \frac{q}{p+q} |\vv^\top T(x)|^3
    < \int_x \frac{pq}{p+q}|\vv^\top T(x)|^2 \cdot q|\vv^\top T(x)|
    \\
    \leq& \left\|\frac{pq}{p+q}\cdot |\vv^\top T|^2\right\|_1 \cdot \big\|q\cdot |\vv^\top T|\big\|_\infty
    = \left(\int_x \frac{pq}{p+q}|\vv^\top T(x)|^2\right) \cdot \sup_x q|\vv^\top T(x)|
    \\
    \leq& \sigma_{\max}(\mH_*) \cdot \TxBdd
    = \TxBdd \kappa_* \sigma_{\min}^*
\end{split}
\end{equation}
where the last step uses Assumption \ref{assump:Tx_bdd}.
Exchanging $p,q$ gives the same bound, hence the factor of 2.


% \input{proofs/not_used/claim_3rd_dev_prev_attempts.tex}

==> proofs/details_lem_radius_progress_hessian/0th.tex <==
% \textbf{Calculating $T_0$}
% 
For $T^{(0)}$, let's first calculate $\int_{x}\frac{q}{2 + \frac{p}{q} + \frac{q}{p}}$:
\begin{equation}
\begin{split}
    =&\int_x \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} 
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{q}{2 + 2\frac{q}{p}}
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{q}{2 + 2\frac{p}{q}}
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} p
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{q^2}{p}
    \\
    \simeq& \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + bx - c\right)
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} - bx + c - 2\log\sqrt{2\pi}\right)
    \\
    \simeq& \exp\left(\frac{b^2}{2}-c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-b)^2}{2}\right)
        %% omit $\frac{1}{2\pi}$ (from $q^2$)
        + \exp\left(\frac{b^2}{2}+c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x+b)^2}{2}\right)
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b} - b} \exp\left(-\frac{x^2}{2}\right)
        + \exp\left(\frac{b^2}{2}+c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}+b} \exp\left(-\frac{x^2}{2}\right)
    \\
    :=& T_{q,1}^{(0)} + T_{q,2}^{(0)}
    \\
    \simeq& \begin{cases}
        \exp(\frac{b^2}{2} - c) + 
        \left(\frac{b}{b^2 + c - \log\sqrt{2\pi}} - \frac{b}{c - \log\sqrt{2\pi} - b^2} \right) \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \geq b
        \\
        \left(\frac{b}{b^2 - c + \log\sqrt{2\pi}} +\frac{b}{b^2 + c - \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \in [-b, b]
        \\
        \exp(\frac{b^2}{2}+c) +
        \left(\frac{b}{b^2 - c + \log\sqrt{2\pi}} +\frac{b}{b^2 + c - \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \leq -b
    \end{cases}
    \\
    =& \begin{cases}
        \exp(\frac{b^2}{2} - c) + 
        \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \geq b
        \\
        \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \in [-b, b]
        \\
        \exp(\frac{b^2}{2}+c) +
        \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} \leq -b
    \end{cases}
    % \simeq& \left(\frac{b}{b^2 - c} +\frac{b}{b^2 + c}\right) \cdot \exp\left(-\frac{c^2}{2b^2}\right)
    % := T_{q,1}^{(0)} + T_{q,2}^{(0)}
    % = \Theta(1/R) \cdot \exp\left(-\frac{c^2}{2b^2}\right)
\end{split}
\end{equation}
% 
The $p_*$ term is calculated similarly:
{
\small
\begin{equation}
\begin{split}
    &\int_x \frac{p_*}{2 + \frac{p}{q} + \frac{q}{p}}
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_*}{2 + 2\frac{q}{p}}
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_*}{2 + 2\frac{p}{q}}
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* p}{q}
    + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* q}{p}
    \\
    =& \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + (R+b)x - c - \frac{R^2}{2}\right)
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + (R-b)x + c - \frac{R^2}{2} - 2\log\sqrt{2\pi}\right)
    \\
    \simeq& \exp\left(\frac{b^2}{2} + bR - c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-R-b)^2}{2}\right)
        %% omit $\frac{1}{2\pi}$ (from $q^2$)
        + \exp\left(\frac{b^2}{2} -bR + c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-R+b)^2}{2}\right)
    \\
    =& \exp\left(\frac{b^2}{2} + bR - c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}-(R+b)} \exp\left(-\frac{x^2}{2}\right)
        + \frac{\exp\left(\frac{b^2}{2} -bR + c\right)}{2\pi} \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}-(R-b)} \exp\left(-\frac{x^2}{2}\right)
    \\
    :=& T_{*,1}^{(0)} + T_{*,2}^{(0)}
    \\
    \simeq& \begin{cases}
        \exp(\frac{b^2}{2} + bR - c) + 
        \left(\frac{b}{b(R-b) - c + \log\sqrt{2\pi}} - \frac{b}{c - \log\sqrt{2\pi}- b(R+b)}\right) \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \geq b
        \\
        \left(\frac{b}{b(R+b) - c + \log\sqrt{2\pi}} + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \in [-b, b]
        \\
        \exp(\frac{b^2}{2}-bR+c) +
        \left(\frac{b}{b(R+b) - c + \log\sqrt{2\pi}} + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \leq -b
    \end{cases}
    \\
    =& \begin{cases}
        \exp(\frac{b^2}{2} + bR - c) + 
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \geq b
        \\
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \in [-b, b]
        \\
        \exp(\frac{b^2}{2}-bR+c) +
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right),
            & \frac{c-\log\sqrt{2\pi}}{b} - R \leq -b
    \end{cases}
    \\
    % \simeq& \left(\frac{b}{b(R+b) - (c-\log\sqrt{2\pi})} + \frac{b}{b(R-b) - (c-\log\sqrt{2\pi})} \right) \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)
    % \\
    % \simeq& \left(\frac{b}{b(R+b) - c} + \frac{b}{b(R-b) - c} \right) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
    % := T_{*,1}^{(0)} + T_{*,2}^{(0)} 
    % = \Theta(1/R) \cdot \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
\end{split}
\end{equation}
}


==> proofs/details_lem_radius_progress_hessian/1st.tex <==

% \textbf{Calculating $T_1$}
For $T^{(1)}$, the $q$ term is:
\begin{equation}
\begin{split}
    &\left|\int_x \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} x\right|
    \leq \max\left\{\int_{x>0} \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} x,\ -\int_{x<0} \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} x\right\}
    \\
    \eqLabel{1}=& \int_{x>0} \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} x
    % \simeq \int_{0< x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{q}{2 + 2\frac{q}{p}} x
    %     + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{q}{2 + 2\frac{p}{q}} x
    \lesssim \int_{0< x < \frac{c-\log\sqrt{2\pi}}{b}} p x
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{q^2}{p} x
    \\
    % \simeq& \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + bx - c\right)
    %     + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} - bx + c - 2\log\sqrt{2\pi}\right)
    % \\
    \lesssim& \exp\left(\frac{b^2}{2}-c\right) \int_{0 < x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-b)^2}{2}\right)x
        %% omit $\frac{1}{2\pi}$ (from $q^2$)
        + \exp\left(\frac{b^2}{2}+c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x+b)^2}{2}\right)x
    \\
    % :=& T_{q,1}^{(1)} + T_{q,2}^{(1)}
    % \\
    =& \exp\left(\frac{b^2}{2}-c\right) \left[\int_{-b < x < \frac{c-\log\sqrt{2\pi}}{b} - b} \exp\left(-\frac{x^2}{2}\right)x
            + b\int_{-b < x < \frac{c-\log\sqrt{2\pi}}{b} - b} \exp\left(-\frac{x^2}{2}\right)\right]
        \\
        &\ + \exp\left(\frac{b^2}{2}+c\right) \left[\int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}+b} \exp\left(-\frac{x^2}{2}\right)x
            - b\int_{x \geq \frac{c-\log\sqrt{2\pi}}{b} + b} \exp\left(-\frac{x^2}{2}\right)\right]
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \left[-\exp\left(-\frac{x^2}{2}\right)\right]_{-b}^{\frac{c-\log\sqrt{2\pi}}{b}-b}
        + \exp\left(\frac{b^2}{2}+c\right) \left[-\exp\left(-\frac{x^2}{2}\right)\right]_{\frac{c-\log\sqrt{2\pi}}{b}+b}^{\infty}
        + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    \\
    % omitting this step (since it's too long)
    % =& \left(b-\frac{c-\log\sqrt{2\pi}}{b}\right) \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right) - b\exp\left(-c\right)
    %     + \left(\frac{c-\log\sqrt{2\pi}}{b}+b\right) \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right)
    %     + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    % \\
    =& \exp(-c) + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    \\
    % \simeq& \exp\left(-\frac{c^2}{2b^2}\right) - \exp\left(-c\right)
        % + \exp\left(-\frac{c^2}{2b^2}\right)
        % + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    % \\
    % \simeq& \exp\left(-\frac{c^2}{2b^2}\right)
    %     + \exp\left(-\frac{c^2}{2b^2}\right)
    %     + b(T_{q,1}^{(0)} - T_{q,2}^{(0)}) 
    % := T_{q,1}^{(1)} + T_{q,2}^{(1)} + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    % \\
    % =& 2 \exp\left(-\frac{c^2}{2b^2}\right)
    %     + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
    % = \Theta(1) \cdot \exp\left(-\frac{c^2}{2b^2}\right)
\end{split}
\end{equation}
where step $\rnum{1}$ is the integration over $x > 0$ is the dominating term for $\param \in \gA$.
% when $c-\log\sqrt{2\pi} \geq 0$.
% The other case (i.e. the $x < 0$ term dominates) has a similar bound of the same order.
% 
The $p_*$ term is calculated similarly (again, consider for now the case where $x<0$ since the other case is analogous):
{
\small
\begin{equation}
\begin{split}
    &\left|\int_x \frac{p_*}{2 + \frac{p}{q} + \frac{q}{p}} x\right|
    \leq \int_{x>0} \frac{p_*}{2 + \frac{p}{q} + \frac{q}{p}} x
    % \simeq \int_{0 < x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_*}{2 + 2\frac{q}{p}}
    %     + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_*}{2 + 2\frac{p}{q}}
    \lesssim \int_{0 < x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* p}{q} x
    + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* q}{p} x
    \\
    % =& \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + (R+b)x - c - \frac{R^2}{2}\right)
    %     + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{x^2}{2} + (R-b)x + c - \frac{R^2}{2} - 2\log\sqrt{2\pi}\right)
    % \\
    \lesssim& \exp\left(\frac{b^2}{2} + bR - c\right) \left[- \exp\left(-\frac{x^2}{2}\right)\right]_{-(R+b)}^{\frac{c-\log\sqrt{2\pi}}{b} - (R+b)}
        %% omit $\frac{1}{2\pi}$ from this term (from $p_* q$)
        + \exp\left(\frac{b^2}{2} -bR + c\right) \left[-\exp\left(-\frac{x^2}{2}\right)\right]_{\frac{c-\log\sqrt{2\pi}}{b}-(R-b)}^{\infty}
        \\
        &\ + (R+b) T_{*,1}^{(0)} + (R-b) T_{*,2}^{(0)}
    \\
    =& \exp\left(-\frac{R^2}{2}-c\right) - \frac{\exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)}{\sqrt{2\pi}}
        %% commenting out a lower order term
        % - \exp\left(-\frac{R^2}{2}-c\right)
        + \frac{\exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)}{\sqrt{2\pi}}
        + (R+b) T_{*,1}^{(0)} + (R-b) T_{*,2}^{(0)}
    \\
    =& \exp\left(-\frac{R^2}{2} - c\right) + (R+b) T_{*,1}^{(0)} + (R-b) T_{*,2}^{(0)}
    % = \Theta(1) \cdot \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
\end{split}
\end{equation}
}


==> proofs/details_lem_radius_progress_hessian/2nd.tex <==
% \textbf{Calculating $T_2$}
% 
For $T^{(2)}$, the $q$ term is:
\begin{equation}
\begin{split}
    &\int_x \frac{q}{2 + \frac{p}{q} + \frac{q}{p}} x^2
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} p x^2
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{q^2}{p} x^2
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-b)^2}{2}\right)x^2
        %% this term should have a factor of $\frac{1}{2\pi}$ from $p_* q$, but we omit it here
        + \exp\left(\frac{b^2}{2}+c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x+b)^2}{2}\right)x^2
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x-b)^2}{2}\right)\left[(x-b) ^2 + 2b(x-b) + b^2\right]
        \\
        &\ + \exp\left(\frac{b^2}{2}+c\right) \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \exp\left(-\frac{(x+b)^2}{2}\right)\left[(x+b)^2 - 2b(x+b) + b^2\right]
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \left[\int_{x < \frac{c-\log\sqrt{2\pi}}{b} - b} \exp\left(-\frac{x^2}{2}\right)x^2
        + 2b\int_{x< \frac{c-\log\sqrt{2\pi}}{b} - b}\exp\left(-\frac{x^2}{2}\right)x\right] + b^2 T_{q,1}^{(0)}
        \\
        &\ + \exp\left(\frac{b^2}{2}+c\right) \left[\int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}+b} \exp\left(-\frac{x^2}{2}\right)x^2
            - 2b\int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}+b} \exp\left(-\frac{x^2}{2}\right)x\right] + b^2 T_{q,2}^{(0)}
    \\
    =& \exp\left(\frac{b^2}{2}-c\right) \left[-\exp\left(-\frac{x^2}{2}\right)x\right]_{-\infty}^{\frac{c-\log\sqrt{2\pi}}{b}-b}
        + \exp\left(\frac{b^2}{2}+c\right) \left[-\exp\left(-\frac{x^2}{2}\right)x\right]_{\frac{c-\log\sqrt{2\pi}}{b}+b}^{\infty}
        \\
        &\ - \frac{4b}{\sqrt{2\pi}}\cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right)
        + (b^2+1) (T_{q,1}^{(0)} + T_{q,2}^{(0)})
    \\
    =& - \frac{2b}{\sqrt{2\pi}}\cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right)
        + (b^2+1) (T_{q,1}^{(0)} + T_{q,2}^{(0)})
    \\
    % \simeq& \left(b-\frac{c}{b}\right) \exp\left(-\frac{c^2}{2b^2}\right) 
    %     %% commenting out a lower order term
    %     % - b\exp\left(-c\right)
    %     + \left(b+\frac{c}{b}\right) \exp\left(-\frac{c^2}{2b^2}\right)
    %     + 2b(T_{q,1}^{(1)} - T_{q,2}^{(1)}) - (b^2-1)(T_{q,1}^{(0)} + T_{q,2}^{(0)})
    % \\
    % \simeq& 2b \exp\left(-\frac{c^2}{2b^2}\right)
    %     + 2b(T_{q,1}^{(1)} - T_{q,2}^{(1)}) - (b^2-1)(T_{q,1}^{(0)} + T_{q,2}^{(0)})
    % \\
    % % =& \left[2b - (b^2-1) \cdot \left(\frac{b}{b^2-c} + \frac{b}{b^2+c}\right)\right] \exp\left(-\frac{c^2}{2b^2}\right)
    % =& \Theta(R) \cdot \exp\left(-\frac{c^2}{2b^2}\right)
\end{split}
\end{equation}
% 
The $p_*$ term is calculated similarly:
{
\small
\begin{equation}
\begin{split}
    &\int_x \frac{p_*}{2 + \frac{p}{q} + \frac{q}{p}} x^2
    \simeq \int_{x < \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* p}{q} x^2
        + \int_{x \geq \frac{c-\log\sqrt{2\pi}}{b}} \frac{p_* q}{p} x^2
    \\
    \simeq& \exp\left(\frac{b^2}{2} + bR - c\right) \int_{x < \frac{c-\log\sqrt{2\pi}}{b}- (R+b)} \exp\left(-\frac{x^2}{2}\right)\left[x^2 + 2(R+b)x + (R+b)^2\right]
        \\
        %% this term should have a factor of $\frac{1}{2\pi}$ from $p_* q$, but we omit it here
        &\ + \exp\left(\frac{b^2}{2} - bR + c\right)\int_{x \geq \frac{c-\log\sqrt{2\pi}}{b} - (R-b)} \exp\left(-\frac{x^2}{2}\right)\left[x^2 + 2(R-b) + (R-b)^2\right]
    \\
    =& \exp\left(\frac{b^2}{2} + bR - c\right) \left[- \exp\left(-\frac{x^2}{2}\right) x\right]_{-\infty}^{\frac{c-\log\sqrt{2\pi}}{b} - (R+b)}
        + \exp\left(\frac{b^2}{2} -bR + c\right) \left[-\exp\left(-\frac{x^2}{2}\right) x\right]_{\frac{c-\log\sqrt{2\pi}}{b}-(R-b)}^{\infty}
        \\
        &\ + \frac{8Rb - 4(c-\log\sqrt{2\pi})}{\sqrt{2\pi}} \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)
        + [(R+b)^2+1] T_{*,1}^{(0)} + [(R-b)^2+1] T_{*,2}^{(0)}
    \\
    =& \frac{2b + 8Rb - 4(c-\log\sqrt{2\pi})}{\sqrt{2\pi}} \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)
    + [(R+b)^2+1] T_{*,1}^{(0)} + [(R-b)^2+1] T_{*,2}^{(0)}
    % \simeq& \left(R+b-\frac{c}{b}\right) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right) 
    %     %% commenting out a lower order term
    %     % - (R+b) \exp\left(-\frac{R^2}{2}-c\right)
    %     - \left(R-b-\frac{c}{b}\right) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right) 
    %     \\
    %     &\ + 2(R+b) T_{*,1}^{(1)} + 2(R-b) T_{*,2}^{(1)}
    %         - (R+b-1) T_{*,1}^{(0)} - (R-b-1) T_{*,2}^{(0)}
    % \\
    % =& \Theta(R) \cdot \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right) 
\end{split}
\end{equation}
}


==> proofs/draft_fix_ngd/G1d_example.tex <==
\textcolor{midgray}{
\textbf{Example on 1d Gaussian}:
consider 1d Gaussian with known variance, i.e. $\bar\delta = [0, b, c]$, and $T(x) = [-\frac{x^2}{2}, x, -1]$.
As before, assume the means are $\theta_q = 0$, $\theta_* = R$ wlog.
\\
Assume $b > 0$ (the $b <0$ case is symmetric), then the first term above can be bounded by:
\begin{equation}
\begin{split}
    T_1 := &\frac{\int_{x:\bar\delta^\top T(x)> 0} \exp\left(\bar\delta^\top T(x)\right) \exp\left(\bar\param^\top T(x)\right) (\vv^\top T(x))^2}
        {\int_{x} \exp\left(\bar\param^\top T(x)\right) (\vv^\top T(x))^2}
    \\
    \overset{(i)}{\leq}& \frac{\int_{x: bx>c} \exp\left(bx-c\right) \exp\left(\bar\param^\top T(x)\right) x^4 dx}
        {\int_{x} \exp\left(\bar\param^\top T(x)\right) x^4 dx}
    \\
    =& \frac{\int_{x: bx>c} \exp\left(-\frac{x^2}{2} + (\frac{R}{2}+b)x - c - \frac{R^2}{8} - \log\sqrt{2\pi}\right) x^4 dx}
        {\int_{x} \exp\left(-\frac{x^2}{2} + \frac{R}{2} - \frac{R^2}{8} - \log\sqrt{2\pi}\right) x^4 dx}
    \\
    =& \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x: bx>c} \exp\left(-\frac{(x-\frac{R}{2}-b)^2}{2}\right) x^4 dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) x^4 dx} 
    \\
    \overset{(ii)}{\leq}& \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x} \exp\left(-\frac{(x-\frac{R}{2}-b)^2}{2}\right) x^4 dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) x^4 dx}  
    \\
    \simeq& \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \frac{\left(\frac{R}{2}+b\right)^4}{(R/2)^4}
    = \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot O\left((1+b/R)^4\right)
\end{split}
\end{equation}
where step $(i)$ increases the value of the expression by picking up the highest order terms in $x$ (i.e. $\vv \parallel \ve_1$),
% \footnote{This assumes $\vv$ is not 0 on the first coordinate; if it is, then we may need to change $x^4$ to $x^2$, which only changes a $\poly(R)$ factor so doesn't matter.}
and step $(ii)$ increases the value by a constant factor.
}

\textcolor{midgray}{
Depending on the value of $b,c$, the RHS can be as small as $O(1)$ and as large as $O(\exp(\|\bar\delta\| R))$.
This means the lower bound should have a matching exponent.
In particular, we have:
\begin{equation}
\begin{split}
    T_1
    \overset{(i)}{\geq}& \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x: x>\frac{b}{c}} \exp\left(-\frac{(x-\frac{R}{2}-b)^2}{2}\right) dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) dx} 
    \\
    \overset{(ii)}{\geq}& \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x: x>\frac{R}{2}+b} \exp\left(-\frac{(x-\frac{R}{2}-b)^2}{2}\right) dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) dx} 
    \\
    =& \frac{1}{2} \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right)
\end{split}
\end{equation}
where step $(i)$ decreases the value of the expression by taking only the constant term (i.e. $\vv \parallel \ve_3$),
step $(ii)$ assumes $\|\bar\delta\| \ll \frac{R}{2}$ s.t. $\frac{b}{c} < \frac{R}{2}+b$.
}

\textcolor{midgray}{
The second term can be bounded similarly:
\begin{equation}
\begin{split}
    %% Upper bound
    T_2 := &\frac{\int_{x:\bar\delta^\top T(x)\leq 0} \exp\left(-\bar\delta^\top T(x)\right) \exp\left(\bar\param^\top T(x)\right) (\vv^\top T(x))^2}
        {\int_{x} \exp\left(\bar\param^\top T(x)\right) (\vv^\top T(x))^2}
    \\
    \overset{(i)}{\leq}& \frac{\int_{x: bx\leq c} \exp\left(-bx+c\right) \exp\left(\bar\param^\top T(x)\right) dx}
        {\int_{x} \exp\left(\bar\param^\top T(x)\right) dx}
    = \exp\left(-\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x: bx\leq c} \exp\left(-\frac{(x-\frac{R}{2}+b)^2}{2}\right) dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) dx} 
    \\
    \overset{(ii)}{\leq}& \exp\left(-\frac{bR}{2} + \frac{b^2}{2} + c\right)
        \cdot \frac{\int_{x} \exp\left(-\frac{(x-\frac{R}{2}+b)^2}{2}\right) dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) dx}  
    = \exp\left(-\frac{bR}{2} + \frac{b^2}{2} + c\right)
    \\
    %% Lower bound
    T_2
    \geq& \exp\left(-\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot \frac{\int_{x: bx\leq c} \exp\left(-\frac{(x-\frac{R}{2}+b)^2}{2}\right) x^4 dx}
        {\int_{x} \exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right) x^4 dx} 
    \geq 0
\end{split}
\end{equation}
}

\textcolor{midgray}{
Hence the ratio is bounded as:
\begin{equation}
\begin{split}
    &\frac{\vv^\top \nabla^2 \Lexp(\tilde\param)\vv}{\vv^\top \mH_* \vv}
    = T_1 + T_2 
    \\
    \in& \left[
        \frac{1}{2}\exp\left(\frac{bR}{2} + \frac{b^2}{2}-c\right),
        \exp\left(\frac{bR}{2} + \frac{b^2}{2} - c\right) \cdot O((1+b/R)^4)
            + \exp\left(-\frac{bR}{2} + \frac{b^2}{2} + c\right)
        \right]
    \\
    \overset{(i)}{=}& \left[\frac{1}{2}\exp\left(\frac{bR}{2} + \frac{b^2}{2}-c\right), \exp\left(\frac{bR}{2} + \frac{b^2}{2}-c\right)\cdot O((1+b/R)^4)\right]
\end{split}
\end{equation}
where step $(i)$ uses the assumption that $b^2 + c^2 \ll R$.
\footnote{Here we assume $b \neq 0$. If $b = 0$, the ratio is bounded simply in $[\exp(-|c|), \exp(|c|)]$, which is a small range since $|c|$ is assumed to be small.}
}

\textcolor{midgray}{
Hence the condition number of $\mH(\tilde\delta)$ is upper bounded by:
\begin{equation}
\begin{split}
    \kappa(\mH(\tilde\delta))
    =& \frac{\sup_{\vu} \vu^\top \mH(\tilde\delta) \vu}
        {\inf_{\vu} \vu^\top \mH(\tilde\delta) \vu}
    = \frac{\sup_{\vu} \vu^\top \mH(\tilde\delta) \vu}{\vv^\top \mH(\tilde\delta)\vv}
        \cdot \frac{\vv^\top \mH(\tilde\delta)\vv}{\inf_{\vu} \vu^\top \mH(\tilde\delta) \vu}
    \\
    \leq& \kappa(\mH_*)
        \cdot \frac{\sup_{\vu} (\vu^\top \mH(\tilde\delta) \vu)/(\vu^\top \mH(\tilde\delta)\vu)}
            {\inf_{\vv} (\vv^\top \mH(\tilde\delta) \vv) / (\vv^\top \mH(\tilde\delta)\vv)} 
    \\
    \leq& \kappa(\mH_*) \cdot O((1+b/R)^4)
    \leq \kappa(\mH_*) \cdot O((1 + \|\bar\delta\|/R)^4)
\end{split}
\end{equation}
}

==> proofs/draft_fix_ngd/sublevel_set_cond.tex <==
\textcolor{RoyalBlue}{// Introducing a new notion of the landscape shape: the condition number of a sublevel set}

\begin{definition}[Condition number of a sublevel set
    \footnote{This definition is similar to \href{https://iwct.sjtu.edu.cn/personal/yingcui/Slides/CO/9-unconstrained-min.pdf}{page 6} of this lecture notes}]
\label{def:sublevel_set_cond}
    Let $C_{\param_*}(\param) := \{\tilde\param: L(\tilde\param) \leq L(\param)\}$ denote the sublevel set of $L$ at $\param$, with the ground truth parameter being $\param_*$.
    The \emph{condition number} $\kappa(C_{\param_*}(\param))$ is defined as the ratio of its maximum and minimum radius,
    i.e. $\kappa(C_{\param_*}(\param)) := \frac{\sup_{\|v\|_2=1} r^2(C_{\param_*}(\param), v)}{\inf_{\|v'\|_2=1} r^2(C_{\param_*}(\param), v')}$, 
    where the radius $r(C_{\param_*}(\param), v)$ is defined as $r(C_{\param_*}(\param), v) := \sup_{\tilde\param \in C_{\param_*}(\param)} v^\top (\tilde\param - \param_*)$.
\end{definition}
%
\begin{assumption}[Bounded condition number of sublevel sets]
\label{assump:sublevel_set_cond}
    $\forall \theta_*, \theta \in \Theta$, $\kappa(C_{\param(\theta_*)})(\param(\theta)) < \paramSubCond$.
\end{assumption}
\textcolor{gray}{\textcolor{orange}{TODO}: can we show that assumption \ref{assump:sublevel_set_cond} holds for the \ENCE~loss?}

In order to have $L(\param_* + \drop\frac{g}{\|g\|}) \leq L(\param)$ for all $\param$ that is at least $\delta$ away from $\param_*$,
it suffices to choose $\drop$ such that the sublevel set of such $\param$ is a superset of the sublevel set of $\param_* + \drop\frac{g}{\|g\|}$ for any $g$.

For any unit vectors $\vv_1, \vv_2$ and constants $c_1, c_2$ such that $L(\param_* + c_1 \vv_1) = L(\param_* + c_2 \vv_2)$ (i.e. $C_{\param_* + c_1\vv_1} = C_{\param_* + c_2\vv_2}$)),
assumption \ref{assump:sublevel_set_cond} guarantees that $\frac{c_1}{c_2} \leq \sqrt{\kappa(C_{\param_*}(\param_*+c_1\vv_1))} \leq \sqrt{\paramSubCond}$.
Therefore setting $\gamma := \frac{\delta}{\sqrt{\paramSubCond}}$ ensures that for any $\param$ that is at least $\delta$ away from $\param_*$, the radius-$\drop$ ball centered at $\param_*$ is a subset of the sublevel set of $\param$,
hence any point in this radius-$\drop$ ball has a smaller loss than $\param$.
\textcolor{gray}{[this is the end of the new proof using $\kappa(C_{\param_*})$.]}

==> proofs/lem_chasm.tex <==
\subsection{Losses and gradients}

Recall that for 1d Gaussian with a known variance of 1, we have parameters $\param_* := \param(\theta_*) = [R, \frac{R^2}{2} + \log\sqrt{2\pi}]$, $\param_q := \param(\theta_q) = [0, \log\sqrt{2\pi}]$,
and sufficient statistics $T(x) = \left[x, -1\right]^\top$.

\textcolor{orange}{TODO: reorganize the proof since the lemma on loss and grad on the line is removed}
% The old lemma \ref{lem:chasm}:
% \begin{lemma}[Loss and gradient in the chasm]
% \label{lem:chasm}
% Consider the 1d Gaussian mean estimation task with parameter $\param(\theta_*), \param(\theta_q)$ and $R := |\theta_* - \theta_q| \gg 1$.
% Consider $\param$ that linearly interpolates between $\param_*$ and $\param_q$, denoted as $\param_t = t\param_* + (1-t)\param_q$. Define $D := tR$.
% Then, for $t\in [\frac{1}{2},1]$ or equivalently $D \in [R/2, R]$, $\param_t$ has an exponentially small loss of $L(\param_t) = \Theta\left(\frac{1}{R}\exp\left(-\frac{R^2}{8}\right)\right)$,
% and an exponentially flat gradient of $\|\nabla_{\param_t}L\|_2 = \Theta\left(\frac{1}{R}\exp\left(-\frac{R^2}{8}\right)\right)$.
% \end{lemma}

For losses and gradients at the optimum and initialization (Proposition \ref{prop:opt_loss}) or in the chasm (Lemma \ref{lem:chasm}), we show a more general result that describes the loss and gradient along the full linear path interpolating $\param_*$ and $\param_q$:

\begin{lemma}[Loss and gradient on the linear path]
\label{lem:loss_grad_line}
Let $P_*, Q$ be in the exponential family.
Let $\tau_*, \tau_q$ be the parameters for $P_*, Q$,
$\tau_* = [\eta_*, c_*] := \left[\theta_*, \frac{\|\theta_*\|^2}{2} + \log\sqrt{2\pi}\right]^\top$,
$\tau_q = [\eta_q, c_q] := \left[\theta_q, \frac{\|\theta_q\|^2}{2} + \log\sqrt{2\pi}\right]^\top$.
Consider $\param$ that linearly interpolates between $\param_*$ and $\param_q$. Denote $\param_t = t\param_* + (1-t)\param_q$ and define $D := tR$, then for $t\in [0,1]$ or equivalently $D \in [0, R]$, the excess risk is:
\begin{equation}
\begin{split}
    c_0 \exp\left(\frac{R^2}{8}\right)L(\param_t) - \frac{\log 2}{\sqrt{2\pi}} \cdot \frac{2}{R} =
    \begin{cases}
        \exp\left(\frac{(D-\frac{R}{2})^2}{2}\right) - c_1,&\ D \in \left[0, \frac{R}{2}\right)
        \\
        \frac{1}{2}, &\ D = \frac{R}{2}
        \\
        c_2, &\ D \in \left(\frac{R}{2}, R\right]
    \end{cases}
\end{split}
\end{equation}
The gradient has coordinates
\begin{equation}
\begin{split}
    c_0^{(1)}\exp\left(\frac{R^2}{8}\right)[\nabla L(\param)]_1 =& -\left(\frac{1}{4} - \frac{1}{2\sqrt{2\pi}}\right) 
    \\
    c_0^{(2)}\exp\left(\frac{R^2}{8}\right)[\nabla L(\param)]_2 =& 
    \begin{cases}
    \exp\Big(\frac{(D - \frac{R}{2})^2}{2}\Big) - c_1', &\ D \in [0, \frac{R}{2})
    \\
    \frac{1}{2}, &\ D = \frac{R}{2}
    \\
    c_2', &\ D \in \left(\frac{R}{2}, R\right]
    \end{cases}
\end{split}
\end{equation}
where $c_0, c_0^{(1)}, c_0^{(2)}\in [1, 2]$, and $c_1, c_2, c_1', c_2' \in O\left(\frac{1}{R}\right)$ satisfy:
\begin{equation}
\begin{split}
    c_1, c_1' \in& \left[\frac{1}{\sqrt{2\pi}}\frac{\frac{R}{2}-D}{(\frac{R}{2}-D)^2 + 1},\ \frac{1}{\sqrt{2\pi}}\frac{1}{\frac{R}{2}-D}\right] 
    \\
    c_2, c_2' \in& \left[\frac{1}{\sqrt{2\pi}}\frac{D-\frac{R}{2}}{(D-\frac{R}{2})^2+1}, \frac{1}{\sqrt{2\pi}}\frac{1}{D-\frac{R}{2}}\right].
\end{split}
\end{equation}
\end{lemma}
Proposition \ref{prop:opt_loss} and Lemma \ref{lem:chasm} are obtained as special cases of Lemma \ref{lem:loss_grad_line} with different values of $t$.

\input{proofs/lem_loss_grad_line_loss}
\input{proofs/lem_loss_grad_line_grad}

==> proofs/lem_ence_step.tex <==
\subsection{Proof of Lemma \ref{lem:ngd_ence_step} (Batch gradient of \ENCE)}

Recall that $d$ is the dimension of the sufficient statistics $T(x)$ (with the augmented dimension for the log partition function),
$\ngrad_t$ denote the normalized population gradient at step $t$,
and $\ngrad_{b,t}$ denote the finite sample version of $\ngrad_t$ evaluated on a batch of size $b$.
\begin{lemma}[Lemma \ref{lem:ngd_ence_step} restated]
\label{lem:ngd_ence_step_restate}
    $\forall \epsilon \in (0,1)$, let $b = \Omega\left(\frac{d}{\epsilon^2}\max\{1, \log (d\epsilon)\}\right)$, then
    $$P\left(\|\ngrad_{t,b} - \ngrad_{t}\| \geq \epsilon \right) \leq \exp\left(-d\ \Omega(\max\{1, \log d\epsilon\})\right).$$
\end{lemma}
\begin{proof}
\textcolor{orange}{[In Progress]}

The gradient can be written as:
\begin{equation}
\begin{split}
    \nabla L
    =& \frac{1}{4} \int_x \sqrt{q}\left(\sqrt{p} - \frac{p_*}{\sqrt{p}}\right) T(x) dx
    = \frac{1}{4} \int_x \sqrt{qp} T(x)dx - \frac{1}{4} \int_x p_*\sqrt{\frac{q}{p}} T(x) dx
    \\
    =& \frac{1}{4} \int_x q \sqrt{\frac{p}{q}}T(x) - \frac{1}{4} \int_x p_*\sqrt{\frac{q}{p}} T(x) dx
    \\
    % =& \frac{Z_{\frac{\theta+\theta_q}{2}}}{\sqrt{Z_\theta Z_{\theta_q}}} \E_{\frac{\theta+\theta_q}{2}}\left[\nabla \log p(x)\right]
        % - \int_x p_*\sqrt{\frac{q}{p}} T(x) dx
    % = \int_x p_*\sqrt{\frac{q}{p}} T(x) dx
\end{split}
\end{equation}
% \textcolor{midgray}{For the first term: $\int_x \sqrt{qp}T(x) = \frac{Z_{\frac{\theta+\theta_q}{2}}}{\sqrt{Z_\theta Z_{\theta_q}}} \E_{\frac{\theta+\theta_q}{2}}\left[\nabla \log p(x)\right] = \frac{Z_{\frac{\theta+\theta_q}{2}}}{\sqrt{Z_\theta Z_{\theta_q}}} \ve_{d+1} \neq 0$ because of the log-partition function.}
% \begin{equation}
% \begin{split}
%     \sqrt{qp} =& \exp\left(\frac{(\param + \param_q)^\top}{2}T(x)\right) = \exp\left(\frac{(\theta+\theta_q)^\top}{2}\tilde{T}(x) - \frac{1}{2}\log Z(\theta) - \frac{1}{2}\log Z(\theta_q)\right)
%     \\
%     =& \frac{Z_{\frac{\theta+\theta_q}{2}}}{\sqrt{Z_\theta Z_{\theta_q}}} \exp\left(\frac{(\theta+\theta_q)^\top}{2} \tilde{T}(x) - \log Z_{\frac{\theta+\theta_q}{2}}\right)
%     = \frac{Z_{\frac{\theta+\theta_q}{2}}}{\sqrt{Z_\theta Z_{\theta_q}}} \cdot p_{\frac{\theta+\theta_q}{2}}(x)
% \end{split}
% \end{equation}

Hence for a size-$2b$ batch with $\{x_i\}_{i\in[b]} \sim P_*$ and $\{x_j\}_{j \in [b]} \sim Q$,
    the batch gradient can be calculated as
% $$\egrad_{t,b} = \frac{1}{4b}\sum_{i \in [b]}\left(\sqrt{\frac{p_t(x_j)}{q(x_j)}} - \sqrt{\frac{q(x_i)}{p_t(x_i)}}\right) T(x_i)$$
$$\egrad_{t,b} = -\frac{1}{4b}\sum_{i \in [b]}\sqrt{\frac{q(x_i)}{p_t(x_i)}} T(x_i) + \frac{1}{4b}\sum_{j \in [b]}\sqrt{\frac{p_t(x_j)}{q(x_j)}} T(x_j)$$
%  \Bnote{we can also evaluate $\left(\sqrt{\frac{p}{q}} - \sqrt{\frac{q}{p}}\right)T(x)$ for $x$ drawn from either $P_*$ or $Q$}

% \textcolor{orange}{\textit{Note}}\textcolor{gray}{: this is not the same as calculating the loss at each point ($\sqrt{\frac{q}{p}}$ or $\sqrt{\frac{p}{q}}$ based on whether the point is from $P_*$ or $Q$) then taking the gradient, which would then give $\nabla \ell(x) = \begin{cases}
%     -\frac{1}{2} \sqrt{\frac{q}{p}} T(x) & x \sim P_* \\
%     \frac{1}{2} \sqrt{\frac{p}{q}} T(x) & x \sim Q
% \end{cases}$.}

We will omit $t$ from the subscript to simplify notations.
By definition, $\ngrad_{b} = \frac{\egrad_{b}}{\|\egrad_{b}\|_2}$, and $\E[\ngrad_{b}] = \ngrad$.
Let $\ngrad_{b,*}$, $\ngrad_{b,q}$ denote the part of $\ngrad_b$ coming from $x$ sampled from $P_*$ and $x$ sampled from $Q$, i.e.
\begin{equation}
\begin{split}
    \ngrad_{b,*} := -\frac{1}{4b\|\egrad_{b}\|_2} \sum_{i \in [b]}\sqrt{\frac{q(x_i)}{p_t(x_i)}} T(x_i),
    ~
    \ngrad_{b,q} := \frac{1}{4b\|\egrad_{b}\|_2}\sum_{j \in [b]}\sqrt{\frac{p_t(x_j)}{q(x_j)}} T(x_j)
\end{split}
\end{equation}
$\ngrad_{*}, \ngrad_{q}$ are defined similarly with the sample average replaced by expectation.

For any unit vector $v \in \R^{d}$,
% \Enote{You should define $\ngrad_{b,*}$ below. Also, are you sure about that integral identity? If it is true, might it require independence? (I'm not saying it's wrong, I just don't immediately see why it should hold. Probably worth explaining).}
% \begin{equation}
% \begin{split}
%     P\left(\left|v^\top (\ngrad_{b} - \ngrad)\right| \geq t \right)
%     = P\left(v^\top (\ngrad_{b} - \ngrad) \geq t\right)
%         + P\left(v^\top (\ngrad_{b} - \ngrad) \leq -t\right)
% \end{split}
% \end{equation}
% \textcolor{midgray}{\textit{Note}: $\ngrad_{b}$ is a bounded random variable, so we should be able to use Hoeffding, as long as we can decompose the gradient into sample averages.
% \textcolor{orange}{Normalization makes decomposing tricky} since
% \begin{equation}
% \begin{split}
%     \ngrad_{b} = \frac{\egrad_{b}}{\|\egrad_{b}\|}
%     = \frac{\egrad_{b,*}}{\|\egrad_{b,*} + \egrad_{b,q}\|}
%          + \frac{\egrad_{b,q}}{\|\egrad_{b,*} + \egrad_{b,q}\|}
% \end{split}
% \end{equation}
% }
\begin{equation}
\begin{split}
    &P\left(\left|v^\top (\ngrad_{b} - \ngrad)\right| \geq t \right)
    = P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*} - (\ngrad_{b,q} - \ngrad_{q}))\right| \geq t \right)
    \\
    \leq& P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*})\right| + \left|v^\top (\ngrad_{b,q} - \ngrad_{q})\right| \geq t \right)
    \\
    \leq& \int_{r=0}^t P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*})\right| > r,~ \left|v^\top (\ngrad_{b,q} - \ngrad_{q})\right| > t-r\right) 
    \\
    \overset{(i)}{=}& \int_{r=0}^t P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*})\right| > r\right) \cdot P\left(\left|v^\top (\ngrad_{b,q} - \ngrad_{q})\right| > t-r\right) 
    \\
    \overset{(ii)}{\leq}& 4\int_{r=0}^t \exp\left(-\frac{br^2}{2} - \frac{b(t-r)^2}{2}\right) dr
    = 4\exp\left(-\frac{bt^2}{4}\right) \int_{r=0}^t \exp\left(-\frac{b}{2}(\sqrt{2}r-t)^2\right) dr
    \\
    \leq& 4t\exp\left(-\frac{bt^2}{4}\right)
    = 4\exp\left(-\frac{bt^2}{4} + \log t\right)
\end{split}
\end{equation}
where $(i)$ uses the independence between $P_*$ and $Q$, and $(ii)$ applies Hoeffding since $|v^\top \ngrad_{b,*}|, |v^\top \ngrad_{*}| \leq 1$ since $v, \ngrad_{b,*}, \ngrad_{*}$ all have norms at most 1, and that $\E\ngrad_{b,*} = \ngrad_{*}$; similarly for $\ngrad_{b,q}, \ngrad_q$.

Let $\{v_1, v_2, ..., v_{d}\}$ be a basis of $\R^{d}$.
Then: \Enote{Not sure the first inequality on the second line is correct? I think it's only true if $\tilde g_b - \tilde g$ is aligned with one of the bases? I think you can fix it by replacing $\epsilon$ with $\epsilon / \sqrt{d}$.}
\begin{equation}
\begin{split}
    &P\left(\|\ngrad_{b} - \ngrad\| \geq \epsilon\right)
    = P\left(\sup_{\|v\|=1} |v^\top (\ngrad_{b} - \ngrad)| \geq \epsilon\right)
    \leq P\left(\sup_{\sum_{[d]}c_i^2 = 1} \sum_{i\in[d]}|c_iv_i^\top (\ngrad_{b} - \ngrad)| \geq \epsilon\right)
    \\
    \leq& P\left(\sup_{i\in[d]}|v_i^\top (\ngrad_{b} - \ngrad)| \geq \epsilon\right)
    \leq \sum_{i\in[d]} P\left(|v_i^\top (\ngrad_{b} - \ngrad)| \geq \epsilon\right)
    \leq 4\exp\left(-\frac{b\epsilon^2}{4} + \log d + \log \epsilon\right)
\end{split}
\end{equation}
Hence $b = \Omega\left(\frac{d}{\epsilon^2}\max\{1, \log (d\epsilon)\}\right)$ guarantees $P\left(\|\ngrad_{b} - \ngrad\| \geq \epsilon\right) \leq \exp\left(-d\Omega(\max\{1, \log d\epsilon\})\right)$.

% \textcolor{gray}{// Bound the unnormalized gradient from $P_*$ first}

% Let $\grad_{*} := \frac{1}{4} \int_x p_*\sqrt{\frac{q}{p}}T(x) dx$,
% and $\egrad_{b,*} := \frac{1}{4b}\sum_{i \in [b]}\sqrt{\frac{q(x_i)}{p_t(x_i)}} T(x_i)$.
% Then for any unit vector $v \in \R^d$,
% \begin{equation}
% \begin{split}
%     &P\left(v^\top \egrad_{b,*} > v^\top \grad_{*} + t\right)
%     = P\left(\exp(sv^\top \egrad_{b,*}) > \exp(sv^\top \grad_{*} + st)\right)
%     \\
%     \overset{(i)}{\leq}& \exp\left(-sv^\top \grad_{*} - st\right)\E_{P_*} \exp(sv^\top \egrad_{b,*})
%     \\
%     \overset{(ii)}{=}& \exp\left(-sv^\top \grad_{*} - st\right)\left[\E_{P_*} \exp\big(\frac{s}{4b}v^\top \sqrt{\frac{q}{p}}T(x)\big)\right]^{b}
%     \\
%     =& \exp\left(-sv^\top \grad_{*} - st\right)\left[\int_x \exp\left(\param_*^\top T(x) + \frac{s}{4b}\sqrt{\frac{q}{p}}v^\top T(x)\right)\right]^{b}
% \end{split}
% \end{equation}
% where $(i)$ is by Markov, and $(ii)$ is because the samples are iid.
% (\textcolor{orange}{todo: $\sqrt{\frac{q}{p}}$})

% \textcolor{gray}{\textit{Note}: if $P = Q$, then
% \begin{equation}
% \begin{split}
%     &\E_{*} \exp\big(\frac{s}{4b}v^\top \sqrt{\frac{q}{p}}T(x)\big) 
%     = \E_{*} \exp\big(\frac{s}{4b}v^\top T(x)\big)
%     \\
%     =& \int_x \exp\left((\theta_* + \frac{s}{4b}v_{:d-1})^\top \tilde{T}(x) - A(\theta_*) - \frac{s}{4b}v_{d}\right)
%     = \exp\left(A(\theta_* + \frac{s}{4b}v_{:d-1}) - A(\theta_*) - \frac{s}{4b}v_{d}\right)
%     \\
%     \overset{(i)}{\leq}& \exp\left(\frac{s^2}{32b^2}\sup_{\tilde{\theta}} \sigma_{\max}(\nabla^2 A(\tilde{\theta}))\|v_{:d-1}\|_2^2 - \frac{s}{4b}v_d\right)
%     = \exp\left(\frac{s^2 \lambda_{\max}}{32b^2}\|v_{:d-1}\|_2^2 - \frac{s}{4b}v_d\right)
%     \\
%     \overset{(ii)}{\leq}& \exp\left(\frac{s^2 \lambda_{\max}}{32b^2} + \frac{s}{4b}\right)
% \end{split}
% \end{equation}
% where $(i)$ uses Taylor expansion, and $(ii)$ is because $v$ is a unit vector.
% }



\textcolor{RoyalBlue}{// Fix the proof}

\textbf{Attempt 1}: write the gradients as the expectation under $\frac{P_*+Q}{2}$. The advantage is that now $\ngrad_{b}, \ngrad$ are both bounded variable, hence we can apply Hoeffding directly.
\begin{equation}
\begin{split}
    \nabla L
    = \frac{1}{4} \int_x q \sqrt{\frac{p}{q}}T(x) - \frac{1}{4} \int_x p_*\sqrt{\frac{q}{p}} T(x) dx
    = \frac{1}{2}\int_x \frac{p_* + q}{2} T(x) \cdot \gamma(p, q, x) dx
\end{split}
\end{equation}
\textit{Challenge}: not sure how $\gamma$ can be independent of $p_*$.

\textbf{Attempt 2}: bound $\ngrad_b$ in terms of the contribution from $P_*$ (i.e. $\ngrad_{b,*}$) and from $Q$ (i.e. $\ngrad_{b,q}$), by first bounding the unnormalized gradients, i.e. $\egrad_{b,*}, \egrad_{b,q}$.
\begin{equation}
\begin{split}
    P\left(\left|v^\top (\ngrad_{b} - \ngrad)\right| \geq t \right)
    \leq& \int_{r=0}^t P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*})\right| > r,~ \left|v^\top (\ngrad_{b,q} - \ngrad_{q})\right| > t-r\right) 
    \\
\end{split}
\end{equation}
% where the first term can be bounded as:
% \begin{equation}
% \begin{split}
%     &P\left(\left|v^\top (\ngrad_{b,*} - \ngrad_{*})\right| > r\right)
%     = P\left(\left|v^\top (\egrad_{b,*} - \grad_{*})\right| > r\|\egrad_b\|\right)
%     = P\left(\left|v^\top (\egrad_{b,*} - \grad_{*})\right|^2 > r^2\|\egrad_b\|^2\right)
%     \\
%     =& P\left(\left|v^\top (\egrad_{b,*} - \grad_{*})\right|^2 > r^2(\|\egrad_{b,*}\|^2 - 2\egrad_{b,*}^\top \egrad_{b,q} + \|\egrad_{b,q}\|^2)\right)
% \end{split}
% \end{equation}
\textit{Challenge}: there is a dependency between samples from $P_*$ and from $Q$.

\textcolor{midgray}{// If we bound the unnormalized gradient instead}

When bounding
\begin{equation}
\begin{split}
    P\left(|v^\top(\egrad_{b,*} - \grad_*)| \geq r\right)
    = P\left(\left|v^\top \left(\frac{1}{b}\sum \sqrt{\frac{q(x_i)}{p(x_i)}}T(x_i) - \E_*\left[\sqrt{\frac{q}{p}}T(x)\right]\right)\right| > r\right)
\end{split}
\end{equation}
\textcolor{gray}{Can we say that $\sqrt{\frac{q}{p}}T(x)$ is sub-gaussian:}
$\forall t > 0$,
\begin{equation}
\begin{split}
    \mu_*
    :=& \E_*\left[\sqrt{\frac{q}{p}}T(x)\right]
    = \int_x \exp\left(\left(\param_* + \frac{\param_q - \param}{2}\right)^\top T(x)\right) T(x) dx
    \\
    =& \frac{Z(\theta_* + \frac{\theta_q - \theta}{2})\sqrt{Z(\theta)}}{Z(\theta_*)\sqrt{Z(\theta_q)}} \cdot \E_{\theta_* + \frac{\theta_q-\theta}{2}}[T(x)]
    \\
\end{split}
\end{equation}
Note that $\theta_* + \frac{\theta_q - \theta}{2}$ may not be in $\Theta$.

$\forall v \in \gS^{d-1}$,
\begin{equation}
\begin{split}
    &\E_*\left[\exp\left(tv^\top(\sqrt{\frac{q}{p}}T(x) - \mu_*)\right)\right]
    = \int_{x} \exp\left(\param_*^\top T(x) + tv^\top(\sqrt{\frac{q}{p}}T(x) - \mu_*)\right)
    \\
    =& \exp(t v^\top \mu_*) \int_x \exp\left(\param_*^\top T(x) + t\sqrt{\frac{q}{p}}v^\top T(x) \right)
\end{split}
\end{equation}
\textit{Challenge}: the expression is a bit too complicated to see what assumption is required.

\textbf{Attempt 3} (\textcolor{orange}{current}):
\begin{equation}
\begin{split}
    &P\left(|v^\top(\ngrad_{b} - \ngrad)| > t\right)
    = P\left(\left|v^\top \left(\frac{\egrad_b}{\|\egrad_b\|} - \frac{\E\egrad_b}{\|\E\egrad_b\|}\right) \right|>t\right)
    \\
    =& P\left(\left|v^\top \left(\frac{\egrad_b}{\|\egrad_b\|} - \E\frac{\egrad_b}{\|\egrad_b\|}
        + \E\frac{\egrad_b}{\|\egrad_b\|} - \frac{\E\egrad_b}{\|\E\egrad_b\|}\right) \right|>t\right)
    \\
    \leq& P\left(\left|v^\top \left(\frac{\egrad_b}{\|\egrad_b\|} - \E\frac{\egrad_b}{\|\egrad_b\|}\right)\right|
        + \underbrace{\left|v^\top\left(\E\frac{\egrad_b}{\|\egrad_b\|} - \frac{\E\egrad_b}{\|\E\egrad_b\|}\right) \right|}_{\gradDiff}>t\right)
    \\
    =& P\left(|v^\top(\ngrad_b - \ngrad)| > t-\gradDiff\right)
    \\
\end{split}
\end{equation}
Note that $v^\top\ngrad_b \in [-1, 1]$.
If we choose $b$ large enough s.t. $\gradDiff < t$, then by Hoeffding,
\begin{equation}
\begin{split}
    &P\left(|v^\top(\ngrad_{b} - \ngrad)| > t\right)
    \leq P\left(\left|v^\top \left(\frac{\egrad_b}{\|\egrad_b\|} - \E\frac{\egrad_b}{\|\egrad_b\|}\right)\right| >
    t - \gradDiff\right)
    \leq \exp\left(-\frac{b^2(t-\gradDiff)}{2}\right)
\end{split}
\end{equation}
It is left to calculate $\gradDiff$ (\textcolor{orange}{todo}).

\textcolor{RoyalBlue}{// Can we bound the expected improvement?}

We would like to mimic the SGD analysis and show that $\E[f(x_{t+1})] \leq f(x_t) - \eta\|\nabla f(x_t)\|_2^2 + \frac{L}{2}\eta^2\E[\|\hat{f}(x_t)\|_2^2]$, where $\E[\|\hat{f}(x_t)\|_2^2]$ is the ``variance'' of the stochastic gradient.
First note that with normalization, the population normalized gradient is no longer the expectation of the batch normalized gradient, i.e. $\ngrad \neq \E[\ngrad_b]$.

\textcolor{gray}{// Point-wise normalized gradients}

The point-wise normalized gradient (which is different from NGD) is decomposable:
Let $\pgrad(x)$ denote the point-wise gradient, with
$\pgrad(x) = \frac{1}{2} q(x)\sqrt{\frac{q(x)}{p(x)}}T(x)
    + \frac{1}{2} p_*(x)\sqrt{\frac{p(x)}{q(x)}}T(x).$
Let $\epgrad(x)$ denote the empirical gradient: let $y \in \{0,1\}$ denote whether a sample $x$ is drawn from $P_*$ ($y=1$) or $Q$ ($y=0$), define
$\epgrad(x) = \frac{1-y}{2} \sqrt{\frac{q(x)}{p(x)}}T(x) + \frac{y}{2} \sqrt{\frac{p(x)}{q(x)}}T(x).$
Then
\begin{equation}
\begin{split}
    \E_{x \sim \frac{P_*+Q}{2}}\left[\frac{\epgrad}{\|\epgrad\|}\right] 
    = \frac{1}{2} \E_{x \sim \frac{P_*+Q}{2}}\left[\frac{T(x)}{\|T(x)\|}\right]
    = \E_{x \sim \frac{P_*+Q}{2}}\left[\frac{\pgrad}{\|\pgrad\|}\right]
\end{split}
\end{equation}
The variance of the point-wise normalized gradient is:
\begin{equation}
\begin{split}
    \E\Big[\Big\|\frac{1}{b}\sum_{i\in[b]}\frac{\epgrad(x_i)}{\|\epgrad(x_i)\|}\Big\|\Big]
    = \frac{b-1}{b}\Big\|\E\Big[\frac{\epgrad(x)}{\|\epgrad(x)\|}\Big]\Big\|^2 + \frac{1}{b}\E\Big[\Big\|\frac{\epgrad(x)}{\|\epgrad(x)\|}\Big\|^2\Big]
\end{split}
\end{equation}


\end{proof}



==> proofs/lem_loss_grad_line_grad.tex <==
\subsubsection{Proof of Lemma \ref{lem:loss_grad_line} part II: Gradient on the linear path}
%
The gradient at $p$ w.r.t. $\param$ is
\begin{equation}
\begin{split}
    \nabla L(\param) =&
    \frac{1}{2}\int_x \frac{q}{p+q} \cdot \left(1 - \frac{p_*}{p}\right)\nabla_{\param'} p
    = \frac{1}{2}\int_x \frac{q}{p+q}(p-p_*)T(x) dx
\end{split}
\end{equation}
When $p=q$, the gradient for 1d Gaussian is:
\begin{equation}
\begin{split}
    \nabla L(\param)
    =& \frac{1}{2} \E_{Q} T(x) - \frac{1}{2}\E_* T(x)
    = \frac{1}{4}\left[\E_Q x, -1\right] - \frac{1}{4}\left[\E_* x, -1\right] 
    = \left[-\frac{R}{8}, 0\right]
\end{split}
\end{equation}
Similar calculations hold for $\param, T(x)$ as well.

Let's first calculate the gradient of the second coordinate of $\param'$:
\begin{equation}
\begin{split}
    2[\nabla L(\param)]_2
    =& \int_x \frac{q}{p+q}(p_*-p) dx
    = \int_x \frac{p_* - p}{1 + \exp\left(D x - \frac{DR}{2}\right)} dx
    \\
    =& \int_x \frac{\exp\left(Rx - \frac{R^2}{2}\right) - \exp\left(Dx - \frac{DR}{2}\right)}{\exp\left(Dx - \frac{DR}{2}\right) + 1} \cdot \exp\left(-\frac{x^2}{2} -\log\sqrt{2\pi}\right)dx
    \\
    =& \int_x \left[\frac{1 + \exp\left(Rx - \frac{R^2}{2}\right)}{1 + \exp\left(Dx - \frac{DR}{2}\right)} - 1\right]q\ dx
    = \int_x \frac{1 + \exp\left(R\left(x - \frac{R}{2}\right)\right)}{1 + \exp\left(D\left(x - \frac{R}{2}\right)\right)} \cdot q dx - 1
\end{split}
\end{equation}

The integration is:
{
\small
\begin{equation}
\begin{split}
    &\int_x \frac{1 + \exp\left(R\left(x - \frac{R}{2}\right)\right)}{1 + \exp\left(D\left(x - \frac{R}{2}\right)\right)} \cdot \frac{\exp\left(-\frac{x^2}{2}\right)}{\sqrt{2\pi}} dx
    = \int_x \frac{1 + \exp\left(Rx\right)}{1 + \exp\left(Dx\right)} \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} dx
    \\
    =& \int_{x \geq 0} \frac{1 + \exp\left(Rx\right)}{1 + \exp\left(Dx\right)} \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} dx
        + \int_{x < 0} \frac{1 + \exp\left(Rx\right)}{1 + \exp\left(Dx\right)} \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} dx
    \\
    \overset{(i)}{\lesssim}& \int_{x \geq 0} \frac{\exp(Rx)}{\exp(Dx)} \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} dx
        + \int_{x < 0} \left(1 + \exp\left(Rx\right)\right) \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} dx
    \\
    =& \int_{x \geq 0} \frac{1}{\sqrt{2\pi}}\exp\left(-\frac{\left(x+\left(D - \frac{R}{2}\right)\right)^2}{2} + \frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right)
        + \int_{x < 0} \frac{\exp\left(-\frac{(x+\frac{R}{2})^2}{2}\right)}{\sqrt{2\pi}} dx
        + \int_{x < 0} \frac{\exp\left(-\frac{(x-\frac{R}{2})^2}{2}\right)}{\sqrt{2\pi}} dx
    \\
    =& \exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right) \cdot P\left(z > D - \frac{R}{2}\right)
        + 1
    \\
    % \overset{(ii)}{=}& \sqrt{2\pi}\left(1 + \exp\left(-\frac{D(R-D)}{2}\right)
        % - \frac{1}{\sqrt{2\pi}} \frac{1}{D - \frac{R}{2}} \exp\left(-\frac{R^2}{8}\right)\right)
\end{split}
\end{equation}
}
where $(i)$ increases the value by at most 2, since $ \frac{1 + \exp\left(Rx\right)}{1 + \exp\left(Dx\right)} \geq  \frac{\exp\left(Rx\right)}{2\exp\left(Dx\right)}$ for $x \geq 0$, and $\frac{1 + \exp(Rx)}{1 + \exp(Dx)} \geq \frac{1+\exp(Rx)}{2}$ for $x < 0$.

Hence 
\begin{equation}
\begin{split}
    [\nabla L(\param)]_2
    = \exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right) \cdot P\left(z > D - \frac{R}{2}\right)
\end{split}
\end{equation}
which can be further simplified depending on the value of $D$:
\begin{itemize}[leftmargin=*]
    \item If $D \in \left[0, \frac{R}{2}\right)$:
    \begin{equation*}
    \begin{split}
        \exp\left(\frac{R^2}{8}\right) [\nabla L(\param)]_2
        =& \exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2}\right) \cdot \left(1 - P\left(z > \frac{R}{2} - D\right)\right)
        \\
        \in& \left[\exp\Big(\frac{(D - \frac{R}{2})^2}{2}\Big) - \frac{1}{\sqrt{2\pi}} \frac{1}{\frac{R}{2}-D},
        \exp\Big(\frac{(D - \frac{R}{2})^2}{2}\Big) - \frac{1}{\sqrt{2\pi}} \frac{\frac{R}{2}-D}{(\frac{R}{2}-D)^2 + 1}\right]
    \end{split}
    \end{equation*}
    
    \item If $D = \frac{R}{2}$:
    $\exp\left(\frac{R^2}{8}\right) [\nabla L(\param)]_2 = \frac{1}{2}\exp\left(-\frac{R^2}{8}\right)$.
    
    \item If $D \in \left(\frac{R}{2}, R\right]$: $\exp\left(\frac{R^2}{8}\right)  [\nabla L(\param)]_2
    \in \left[\frac{1}{\sqrt{2\pi}} \frac{D-\frac{R}{2}}{(D-\frac{R}{2})^2 + 1},\ \frac{1}{\sqrt{2\pi}} \frac{1}{D-\frac{R}{2}}\right]$.
\end{itemize}
% 
% 
The calculation for the gradient at the first coordinate of $\param$ is similar:
\begin{equation}
\begin{split}
    &2[\nabla L(\param)]_1
    = \int_x \frac{q}{p+q}(p-p_*)x dx
    = \int_x \left[1 - \frac{1 + \exp\left(Rx - \frac{R^2}{2}\right)}{1 + \exp\left(Dx - \frac{DR}{2}\right)}\right]qx dx
    \\
    =& -\int_x \frac{1 + \exp\left(R\left(x - \frac{R}{2}\right)\right)}{1 + \exp\left(D\left(x - \frac{R}{2}\right)\right)} \cdot qx dx
    = -\int_x \frac{1 + \exp\left(R\left(x - \frac{R}{2}\right)\right)}{1 + \exp\left(D\left(x - \frac{R}{2}\right)\right)} \cdot \frac{\exp\left(-\frac{x^2}{2}\right)}{\sqrt{2\pi}} xdx
    \\
    \overset{(i)}{\leq}& -\frac{1}{2} \int_{x \geq 0} \frac{\exp(Rx)}{\exp(Dx)} \cdot \exp\left(-\frac{(x+R/2)^2}{2}\right) xdx
        - \frac{1}{2}\int_{x < 0} \left(1 + \exp\left(Rx\right)\right) \cdot \frac{\exp\left(-\frac{(x+R/2)^2}{2}\right)}{\sqrt{2\pi}} xdx
    \\
    =& -\frac{1}{2}\exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right) \cdot \int_{x \geq 0} \frac{\exp\left(-\frac{\left(x + \left(D - \frac{R}{2}\right)\right)^2}{2}\right)}{\sqrt{2\pi}} xdx
        \\
        &\ - \frac{1}{2\sqrt{2\pi}} \int_{x < 0} \exp\left(-\frac{(x+R/2)^2}{2}\right) xdx
        - \frac{1}{2\sqrt{2\pi}} \int_{x < 0} \exp\left(-\frac{(x-R/2)^2}{2}\right) xdx
    \\
    =& -\frac{1}{2}\exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right) \cdot \left[-\exp\left(-\frac{\left(x + \left(D - \frac{R}{2}\right)\right)^2}{2}\right)\right]_0^{\infty}
         - \frac{1}{2\sqrt{2\pi}} \left[-\exp\left(-\frac{(x+R/2)^2}{2}\right)\right]_{-\infty}^{0}
         \\
         &\ - \frac{1}{2\sqrt{2\pi}}\left[-\exp\left(-\frac{(x-R/2)^2}{2}\right)\right]_{-\infty}^{0}
    \\
    =& -\frac{1}{2} \exp\left(\frac{\left(D - \frac{R}{2}\right)^2}{2} - \frac{R^2}{8}\right) \cdot \exp\left(-\frac{\left(D - \frac{R}{2}\right)^2}{2}\right)
        + \frac{1}{\sqrt{2\pi}}\exp\left(-\frac{R^2}{8}\right)
    \\
    =& -\left(\frac{1}{2} - \frac{1}{\sqrt{2\pi}}\right) \exp\left(-\frac{R^2}{8}\right)
\end{split}
\end{equation}
where $(i)$ increases the value by at most 2.


==> proofs/lem_loss_grad_line_loss.tex <==
\subsubsection{Proof of Lemma \ref{lem:loss_grad_line} part I: Loss on the linear path}
% 
Since $\param$ linearly interpolates between $\param_q$ and $\param_*$, let's parameterize it as
\begin{equation}
\begin{split}
    \param_t :=&\ t\param_* + (1-t)\param_q
    = \left[t\theta_*+(1-t)\theta_q,  \frac{t\|\theta_*\|^2 + (1-t)\|\theta_q\|^2}{2} + \log\sqrt{2\pi}\right]^\top
    \\
    =& \left[t\theta_*,  \frac{t\|\theta_*\|^2 }{2} + \log\sqrt{2\pi}\right]^\top
\end{split}
\end{equation}
for $t \in [0, 1]$.

The loss at $\param_t$ is
{\small
\begin{equation}
\begin{split}
    &L(\param_t)
    = \frac{1}{2}\int_x p_* \log\left(1 + \frac{q}{p}\right) + \frac{1}{2}\int_x q \log\left(1 + \frac{p}{q}\right)
    \\
    =& \frac{1}{2}\int_x p_*\log\left(1 + \exp\left(t(\theta_q - \theta_*)x + \frac{t(\|\theta_*\|^2 - \|\theta_q\|^2)}{2}\right)\right)
        + \frac{1}{2}\int_x q\log\left(1 + \exp\left(-t(\theta_q - \theta_*)x - \frac{t(\|\theta_*\|^2 - \|\theta_q\|^2)}{2}\right)\right)
    \\
    =& \frac{1}{2}\int_x p_*\log\left(1 + \exp\left(tR\left(\frac{R}{2}-x\right)\right)\right)
        + \frac{1}{2}\int_x q\log\left(1 + \exp\left(-tR\left(\frac{R}{2}-x\right)\right)\right)
    \\
    =& \frac{1}{2}\int_{x} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(x-R)^2}{2}\right)\log\left(1 + \exp\left(tR\left(\frac{R}{2}-x\right)\right)\right)
        + \frac{1}{2}\int_x q\log\left(1 + \exp\left(-tR\left(\frac{R}{2}-x\right)\right)\right)
    \\
    \overset{(i)}{=}& \frac{1}{2}\int_{x'} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(x')^2}{2}\right)\log\left(1 + \exp\left(-tR\left(\frac{R}{2}-x'\right)\right)\right)
        + \frac{1}{2}\int_x q\log\left(1 + \exp\left(-tR\left(\frac{R}{2}-x\right)\right)\right)
    \\
    =& \int_x q\log\left(1 + \exp\left(-tR\left(\frac{R}{2}-x\right)\right)\right)
    \\
    \overset{(ii)}{\lesssim}& \int_{x \leq \frac{R}{2}} q \cdot \exp\left(-tR\left(\frac{R}{2}-x\right)\right)
        + \int_{x \geq \frac{R}{2}} q\log\left(2\cdot \exp\left(-tR\left(\frac{R}{2}-x\right)\right)\right)
    \\
    =& \exp\left(-\frac{t(1-t)R^2}{2}\right) \int_{x \leq \frac{R}{2}} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(x-tR)^2}{2}\right)
        + \left(\log 2- \frac{tR^2}{2}\right) \cdot \int_{x \geq \frac{R}{2}} q
        + tR\int_{x \geq \frac{R}{2}} qx
    \\
    \overset{(iii)}{\lesssim}& \exp\left(-\frac{t(1-t)R^2}{2}\right) \int_{x \leq \frac{R}{2}} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(x-tR)^2}{2}\right)
        + \left(\log 2- \frac{tR^2}{2}\right) \frac{1}{\sqrt{2\pi}} \frac{2}{R}\exp\left(-\frac{R^2}{8}\right)
        + \frac{tR}{\sqrt{2\pi}}\left[-\exp\left(-\frac{x^2}{2}\right)\right]_{\frac{R}{2}}^\infty
    \\
    =& \underbrace{\exp\left(-\frac{t(1-t)R^2}{2}\right) \int_{x \leq \frac{R}{2}} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(x-tR)^2}{2}\right)}_{T_1}
    + \frac{\log 2}{\sqrt{2\pi}}\cdot \frac{2}{R}\exp\left(-\frac{R^2}{8}\right) 
\end{split}
\end{equation}
}

where $(i)$ applies a change of variable $x' = R - x$;
$(ii)$ increases the value by at most 2 since $\log(1+x) \geq \frac{1}{2}x$ for $x\in [0,1]$, and $\log(1+x) \geq \frac{1}{2}\log(2x)$ for $x \geq 1$;
$(iii)$ increases the value by at most $\frac{R^2+4}{R^2}$, which is less than $2$ since $R$ is assumed to be sufficiently large.

%The first term $T_1$ takes different values depending on the value of $t$. 
Let $D := tR$. Then, $T_1$ can be rewritten as:
% $\exp\left(-\frac{D(R-D)}{2}\right)\int_{x\leq \frac{R}{2}}\frac{1}{\sqrt{2\pi}}\exp\left(-\frac{(x - D)^2}{2}\right)$, whose value is:
\begin{equation}
\begin{split}
    T_1 = \exp\left(-\frac{D(R-D)}{2}\right)\int_{x\leq \frac{R}{2}}\frac{1}{\sqrt{2\pi}}\exp\left(-\frac{(x - D)^2}{2}\right)
    = \exp\left(\frac{(D-\frac{R}{2})^2}{2} - \frac{R^2}{8}\right) \cdot P\left(z \leq \frac{R}{2} - D\right)
\end{split}
\end{equation}
We will distinguish several cases according to what $D$ is: 
\begin{itemize}[leftmargin=*]
    \item If $D \in \left[0, \frac{R}{2}\right)$:
    \begin{equation}
    \begin{split}
        &P\left(z \leq \frac{R}{2} - D\right) = 1 - P\left(z \geq \frac{R}{2} - D\right) \leq 1 - \frac{1}{\sqrt{2\pi}}\frac{\frac{R}{2}-D}{(\frac{R}{2}-D)^2+1}\exp\left(-\frac{(D-\frac{R}{2})^2}{2}\right)
        \\
        \Rightarrow&
        T_1 \leq \left(\exp\Big(\frac{(D-\frac{R}{2})^2}{2}\Big) - \frac{1}{\sqrt{2\pi}}\frac{\frac{R}{2}-D}{(\frac{R}{2}-D)^2+1}\right) \cdot \exp\left(- \frac{R^2}{8}\right)
    \end{split}
    \end{equation}
    Similarly, $T_1 \geq \left(\exp\Big(\frac{(D-\frac{R}{2})^2}{2}\Big) - \frac{1}{\sqrt{2\pi}}\frac{1}{\frac{R}{2}-D}\right) \cdot \exp\left(- \frac{R^2}{8}\right)$

    \item If $D = \frac{R}{2}$: $T_1 = \frac{1}{2}\exp\left(\frac{(D-\frac{R}{2})^2}{2} - \frac{R^2}{8}\right) = \frac{1}{2}\exp\left(-\frac{R^2}{8}\right)$.
    
    \item If $D \in \left(\frac{R}{2}, R\right]$:
    \begin{equation}
    \begin{split}
        &P\left(z \leq \frac{R}{2} - D\right) = P\left(z \geq D - \frac{R}{2}\right) \leq \frac{1}{\sqrt{2\pi}}\frac{1}{D-\frac{R}{2}}\exp\left(-\frac{(D-\frac{R}{2})^2}{2}\right)
        \\
        \Rightarrow&
        T_1 \leq \frac{1}{\sqrt{2\pi}}\frac{1}{D-\frac{R}{2}}\exp\left(-\frac{R^2}{8}\right)
    \end{split}
    \end{equation}
    Similarly, $T_1 \geq \frac{1}{\sqrt{2\pi}}\frac{D-\frac{R}{2}}{(D-\frac{R}{2})^2+1}\exp\left(-\frac{R^2}{8}\right)$.
\end{itemize}

Hence the loss evaluates to:
\begin{equation}
\begin{split}
    \exp\left(\frac{R^2}{8}\right)L(\param) =
    \begin{cases}
        \exp\left(\frac{(D-\frac{R}{2})^2}{2}\right) + \frac{\log 2}{\sqrt{2\pi}} \cdot \frac{2}{R} - c_1,&\ D \in \left[0, \frac{R}{2}\right)
        \\
        \frac{1}{2} + \frac{\log 2}{\sqrt{2\pi}} \cdot \frac{2}{R}, &\ D = \frac{R}{2}
        \\
        c_2 + \frac{\log 2}{\sqrt{2\pi}} \cdot \frac{2}{R}, &\ D \in \left(\frac{R}{2}, R\right]
    \end{cases}
\end{split}
\end{equation}
where constants $c_1, c_2$ satisfy:
\begin{equation}
\begin{split}
    c_1 \in& \left[\frac{1}{\sqrt{2\pi}}\frac{\frac{R}{2}-D}{(\frac{R}{2}-D)^2 + 1},\ \frac{1}{\sqrt{2\pi}}\frac{1}{\frac{R}{2}-D}\right]
    \\
    c_2 \in& \left[\frac{1}{\sqrt{2\pi}}\frac{D-\frac{R}{2}}{(D-\frac{R}{2})^2+1}, \frac{1}{\sqrt{2\pi}}\frac{1}{D-\frac{R}{2}}\right].
\end{split}
\end{equation}
\vspace{1em}

==> proofs/lem_nce_exp_kappa.tex <==
% \subsection{Proof of Lemma \ref{lem:nce_exp_kappa}}

% We will first prove Lemma \ref{lem:nce_exp_kappa}, whose calculations will be useful for proving Theorem \ref{thm:nce_exp_ngd}.

% \begin{lemma}[Lemma \ref{lem:nce_exp_kappa} restated]
% \label{lem:nce_exp_kappa_restated}
% Let $\lambda_{\max}, \lambda_{\min}$ be as defined in assumption \ref{assump:Fisher_bdd}.
% Then, for any $P_*, Q$ under assumption \ref{assump:param_norm_bdd}-\ref{assump:Tx_2nd3rd}, the condition number of the \ENCE Hessian at the optimum is bounded by 
% $\kappa_* \leq \frac{\lambda_{\max}}{\lambda_{\min}}$.
% \end{lemma}

% \begin{proof}We first write down the loss, gradient and Hessian of \ENCE~ for the exponential family:
\begin{equation}\label{eq:ence_loss_grad_hessian}
\begin{split}
    \Lexp(P)
    =& \frac{1}{2}\int_x p_*\sqrt{\frac{q}{p}} + \frac{1}{2}\int_x q \sqrt{\frac{p}{q}}
    \\
    \nabla \Lexp(P)
    =& \frac{1}{4}\int_x \sqrt{q}\left(\sqrt{p} - \frac{p_*}{\sqrt{p}}\right) \nabla\log p
    \\
    \nabla^2 \Lexp(P)
    =& \frac{1}{4} \int_{x} \sqrt{q}\left(\sqrt{p} - \frac{p_*}{\sqrt{p}}\right) \cdot \nabla^2 \log p
        + \frac{1}{8} \int_x \sqrt{q} \left(\sqrt{p} + \frac{p_*}{\sqrt{p}}\right)\nabla \log p (\nabla \log p)^\top 
    \\
    =& \frac{1}{8} \int_x \sqrt{q} \left(\sqrt{p} + \frac{p_*}{\sqrt{p}}\right)\nabla \log p (\nabla \log p)^\top
    \\
    =& \frac{1}{8} \int_x p_*\sqrt{\frac{q}{p}}T(x)T(x)^\top
        + \frac{1}{8} \int_x q \sqrt{\frac{p}{q}} T(x)T(x)^\top 
    \\
\end{split}
\end{equation}

Note that the Hessian is always PSD, which means $\Lexp$ is convex in the parameters of the exponential family.
% Moreover, the Hessian at $P = P_*$ is:
% \begin{equation}
% \begin{split}
%     \mH_* := \nabla^2 L(P_*)
%     = \frac{1}{4}\int_x \sqrt{p_*q} \nabla \log p (\nabla \log p)^\top 
% \end{split}
% \end{equation}
% Recall that $\theta_*, \theta_q, \tilde{T}$ denote the parameters and sufficient statistics without the partition function coordinate, and $\param_*, \param_q, T$ denote the extended version with the partition function, e.g. $\param_{*} = [\theta_*, \log Z(\theta_*)]$, $T(x) = [\tilde{T}(x), -1]$.
% Then, we can rewrite $\mH_*$ as:
% \begin{equation}
% \begin{split}    
%     \mH_*
%     =& \frac{1}{4}\int_x \sqrt{p_*q}T(x)T(x)^\top
%     = \frac{1}{4}\int_x \exp\left(\frac{(\param_* + \param_q)^\top}{2} T(x)\right) T(x)T(x)^\top 
%     \\
%     =& \frac{1}{4}\int_x \exp\left(\frac{(\theta_* + \theta_q)^\top}{2} \tilde{T}(x) - \frac{1}{2}\log Z(\theta_*) - \frac{1}{2}\log Z(\theta_q)\right) T(x)T(x)^\top 
%     % = \frac{1}{4}\exp(c_Z)\int_x \exp\left(\big(\frac{\param_* + \param_q}{2} + c_Z\ve_{d+1}\big)^\top T(x)\right) T(x) T(x)^\top dx
%     \\
%     =&  \frac{1}{4} \underbrace{\frac{Z\left(\frac{\theta_* +\theta_q}{2}\right)}{\sqrt{Z(\theta_*)Z(\theta_q)}}}_{B(P_*, Q)} \int_x \frac{\exp\left(\big(\frac{\theta_* + \theta_q}{2}\big)^\top \tilde{T}(x)\right)}{Z\left(\frac{\theta_* +\theta_q}{2}\right)} T(x) T(x)^\top dx
%     = \frac{B(P_*, Q)}{4}\E_{\frac{\theta_*+\theta_q}{2}}[TT^\top]
%     \\
%     % =& \frac{1}{4} \underbrace{\frac{Z\left(\frac{\theta_* +\theta_q}{2}\right)}{\sqrt{Z(\theta_*)Z(\theta_q)}}}_{B} \E_{\frac{\theta_*+\theta_q}{2}}[TT^\top]
% \end{split}
% \end{equation}
% Since $\frac{\theta_* + \theta_q}{2} \in \Theta$,
% we have $\lambda_{\min}\mI \preceq \E_{\frac{\theta_*+\theta_q}{2}}[TT^\top] \preceq \lambda_{\max}\mI$ by Assumption \ref{assump:Fisher_bdd}. The Lemma hence follows. 

% Note that even though $B(P_*, Q)$ can be exponentially small or large, the condition number is unaffected.
% \end{proof}

==> proofs/lem_nce_sigma_min.tex <==
% \subsubsection{Proof of Lemma \ref{lem:nce_hessian_sigma_min}}
\subsubsection{Calculations for minimum singular values (draft; to be removed)}

The Hessian at $(b,c)$ is:
\begin{equation}\label{eq:nce_hessian_expression}
\begin{split}
    \nabla^2 L 
    =& \frac{1}{2} \int_x \frac{(p_*+q)pq}{(p+q)^2} T(x)T(x)^\top dx
    = \frac{1}{2} \int_x \frac{p_* + q}{2 + \frac{p}{q} + \frac{q}{p}} \cdot \begin{bmatrix}x^2 & -x \\ -x & 1\end{bmatrix}
    := \frac{1}{2} \begin{bmatrix}
        T^{(2)} & -T^{(1)} \\ -T^{(1)} & T^{(0)}
    \end{bmatrix}
    \\
\end{split}
\end{equation}
$\sigma_{\min}(\nabla^2 L)$ can be lower bounded as:
\begin{equation}\label{eq:nce_sigma_min_lb}
\begin{split}
    \sigma_{\min}(\nabla^2 L)
    = \frac{\det(\nabla^2 L)}{\sigma_{\max}(\nabla^2 L)}
    \geq \frac{T^{(2)} T^{(0)} - (T^{(1)})^2}{T^{(2)} + |T^{(1)}|}
    % = \frac{\Theta(1) \cdot E^2}{\Theta(R) \cdot E}
    % = \Theta(1/R) \cdot E
    % = \Theta(1/R) \exp\left(-\frac{\kappa(b,c) \cdot R^2}{8}\right)
\end{split}
\end{equation}
We now calculate $T^{(0)}$ and $T^{(2)}$, and an upper bound of $T^{(1)}$.
We show the calculations for $b > 0$; the $b< 0$ case is analogous.

% It can be shown that
% \begin{equation}
% \begin{split}
%     T^{(0)} =& \Theta(1/R) \exp\left(-\frac{c^2}{2b^2}\right)
%         + \Theta(1/R) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
%     \\
%     T^{(1)} =& \Theta(1) \exp\left(-\frac{c^2}{2b^2}\right)
%         + \Theta(1) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
%     \\
%     T^{(2)} =& \Theta(R) \exp\left(-\frac{c^2}{2b^2}\right)
%         + \Theta(R) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
% \end{split}
% \end{equation}

\input{proofs/details_lem_radius_progress_hessian/0th}
\input{proofs/details_lem_radius_progress_hessian/1st}
\input{proofs/details_lem_radius_progress_hessian/2nd}

Recall that we have used $b>0, c-\log\sqrt{2\pi}$ in previous calculations.
Denote
$E_1 := \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right)$,
$E_2 := \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)$,
then 
\begin{equation}
\begin{split}
    T_0 \simeq&\ T_{q,1}^{(0)} + T_{q,2}^{(0)} + T_{*,1}^{(0)} + T_{*,2}^{(0)}
        := T_q^{(0)} + T_*^{(0)}
    \\
    |T_1| \leq&\ \exp(-c) + \exp\left(-\frac{R^2}{2} - c\right)
        + R T_{*}^{(0)} 
        + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
        + b(T_{*,1}^{(0)} - T_{*,2}^{(0)})
        \\
        \simeq& \exp(-c)
        + R T_{*}^{(0)} 
        + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
        + b(T_{*,1}^{(0)} - T_{*,2}^{(0)}) 
    \\
    T_2
    \simeq& \underbrace{- \frac{2b}{\sqrt{2\pi}}\cdot E_1
    + \frac{2b + 8Rb - 4(c-\log\sqrt{2\pi})}{\sqrt{2\pi}} E_2}_{:= E}
        \\
        &\ + (b^2+1) T_{q}^{(0)}
        + (R^2 + b^2 + 1) T_{*}^{(0)}
        - 2Rb (T_{*,1}^{(0)} - T_{*,2}^{(0)})
    \\
    =& b^2 T_q + (T_q + T_*) + (R-b)^2 T_{*,1} + (R+b)^2 T_{*,2} - \frac{2b}{\sqrt{2\pi}} E_1 + \frac{2b + 8Rb - 4(c-\log\sqrt{2\pi})}{\sqrt{2\pi}} E_2
\end{split}
\end{equation}
%
Omitting the superscript $\{(0)\}$ for convenience, we have:
{
\small 
\begin{equation}
\begin{split}
    T_2 T_0 - (T_1)^2
    \geq& (T_q + T_*) E + T_q^2 + 4b^2 T_{q,1}T_{q,2}
        + T_*^2 + 4b^2 T_{*,1} T_{*,2}
        - 3Rb(T_{*,1}^2 - T_{*,2}^2)
        \\
        &\ + (R^2 + 2) T_* T_q + 4b^2 (T_{q,1}T_{*,2} + T_{q,2} T_{*,1})
        - 2Rb(T_{q,1} T_{*,1} - T_{q,2}T_{*,2})
        \\
        &\ - 2\exp(-c)b (T_{q,1} - T_{q,2} + T_{*,1} - T_{*,2})
        - \exp(-2c) - 2\exp(-c) R T_*
\end{split}
\end{equation}
% 
\begin{equation}
\begin{split}
    &T_2 + |T_1|
    = - \frac{2b}{\sqrt{2\pi}}\cdot E_1
        + \frac{2b + 8Rb - 4(c-\log\sqrt{2\pi})}{\sqrt{2\pi}} E_2
        + \exp(-c) + \exp\left(-\frac{R^2}{2} - c\right)
        \\
        &\ + (R^2 + b^2 + R + 1) T_*^{(0)} + (b^2+1) T_q^{(0)}
        + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
        - (2R-1)b (T_{*,1}^{(0)} - T_{*,2}^{(0)})
    \\
    \simeq& - \frac{2b}{\sqrt{2\pi}}\cdot E_1
        + \frac{2Rb - (c-\log\sqrt{2\pi})}{\sqrt{2\pi}} \cdot 4E_2
        + \exp(-c)
        \\
        &\ + (R^2 + b^2) T_*^{(0)} + (b^2+1) T_q^{(0)}
        + b(T_{q,1}^{(0)} - T_{q,2}^{(0)})
        - 2Rb (T_{*,1}^{(0)} - T_{*,2}^{(0)})
\end{split}
\end{equation}
}

\textcolor{RoyalBlue}{// Copy over for convenience}
\begin{equation}
\begin{split}
    T_q \simeq& \begin{cases}
        \exp(\frac{b^2}{2} - c) + \frac{b}{b^2 - c + \log\sqrt{2\pi}} E_1 
            + \frac{b}{b^2 + c - \log\sqrt{2\pi}} E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \geq b
        \\
        \frac{b}{b^2 - c + \log\sqrt{2\pi}} E_1
            + \frac{b}{b^2 + c - \log\sqrt{2\pi}} E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \in [0, b]
        \\
        % \frac{b}{b^2 - c + \log\sqrt{2\pi}} E_1
        % + \exp(\frac{b^2}{2}+c) + \frac{b}{b^2 + c - \log\sqrt{2\pi}}E_1,
        %     & \frac{c-\log\sqrt{2\pi}}{b} \leq -b
    \end{cases}
    \\
    =& \begin{cases}
        \exp(\frac{b^2}{2} - c) + 
        \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \geq b
        \\
        \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \in [0, b]
        \\
        % \exp(\frac{b^2}{2}+c) +
        % \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
        %     & \frac{c-\log\sqrt{2\pi}}{b} \leq -b
    \end{cases}
    \\
    =& \exp\Big(\frac{b^2}{2}-c\Big) \cdot \I\{c-\log\sqrt{2\pi} \geq b^2\}
        + \frac{2b^3}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1
    \\
    %%%
    %%%
    T_* \simeq& \begin{cases}
        \exp(\frac{b^2}{2} + bR - c) +  \frac{b}{b(R+b) - c + \log\sqrt{2\pi}} E_2
        + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}} E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \geq b
        \\
        \frac{b}{b(R+b) - c + \log\sqrt{2\pi}} E_2 + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}} E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \in [-b, b]
        \\
        \frac{b}{b(R+b) - c + \log\sqrt{2\pi}} E_2
        + \exp(\frac{b^2}{2}-bR+c) + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}} E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \leq -b
    \end{cases}
    \\
    =& \begin{cases}
        \exp(\frac{b^2}{2} + bR - c) + 
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} \geq R+b
        \\
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} \in [R-b, R+b]
        \\
        \exp(\frac{b^2}{2}-bR+c) +
        \frac{2(Rb-c+\log\sqrt{2\pi})b}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} \in [0, R-b]
    \end{cases}
    \\
\end{split}
\end{equation}
%%
\begin{equation}
\begin{split}
    T_{q,1} - T_{q,2}
    \simeq& \begin{cases}
        \exp(\frac{b^2}{2} - c) + 
        \frac{2b(c-\log\sqrt{2\pi})}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \geq b
        \\
        \frac{2b(c-\log\sqrt{2\pi})}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \in [-b, b]
        \\
        -\exp(\frac{b^2}{2}+c) +
        \frac{2b(c-\log\sqrt{2\pi})}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1,
            & \frac{c-\log\sqrt{2\pi}}{b} \leq -b 
    \end{cases}
    \\
    T_{*,1} - T_{*,2}
    \simeq& \begin{cases}
        \exp(\frac{b^2}{2} + bR - c) - 
        \frac{2b^3}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \geq b
        \\
        -\frac{2b^3}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \in [-b, b]
        \\
        -\exp(\frac{b^2}{2}-bR+c) -
        \frac{2b^3}{(b(R-b)-c+\log\sqrt{2\pi}) (b(R+b)-c+\log\sqrt{2\pi})} \cdot E_2,
            & \frac{c-\log\sqrt{2\pi}}{b} - R \leq -b
    \end{cases} 
\end{split}
\end{equation}

When $\frac{c - \log\sqrt{2\pi}}{b} = \frac{R}{2}$, $E_1 = E_2 = \exp\left(-\frac{R^2}{8}\right)$.

When $\frac{c-\log\sqrt{2\pi}}{b} < \frac{R}{2}$, $E_1 > E_2$,
\begin{equation}
\begin{split}
    T_0 \simeq&\ T_q
    \\
    |T_1| \leq&\ \exp(-c) + b(T_{q,1} - T_{q,2})
    \\
    T_2
    \simeq& (b^2+1) T_q - \frac{2b}{\sqrt{2\pi}} E_1
\end{split}
\end{equation}
%
\begin{equation}
\begin{split}
    &T_2 T_0 - |T_1|^2
    \\
    \geq& (b^2+1)T_q^2 - \frac{2b}{\sqrt{2\pi}}E_1 T_q - \exp(-2c) - b^2(T_{q,1}-T_{q,2})^2 - 2\exp(-c)b(T_{q,1}-T_{q,2})
    \\
    \simeq& \begin{cases}
        (b^2+1) \exp\left(b^2-2c\right) - \exp(-2c) - b^2 \exp(b^2-2c) - 2b\exp(\frac{b^2}{2}-2c),
        & c-\log\sqrt{2\pi} \geq b^2
        \\
        (b^2+1) \Theta(b^2) E_1^2 - \frac{2b}{\sqrt{2\pi}} E_1^2 - b^2 \Theta(b^2) E_1^2,
        & c-\log\sqrt{2\pi} < b^2
    \end{cases}
    \\
    =& \begin{cases}
        \left[\exp(b^2) - 1 - 2b\exp(\frac{b^2}{2})\right] \cdot \exp(-2c),
        & c-\log\sqrt{2\pi} \geq b^2
        \\
        \Theta(b^4) E_1^2, & c-\log\sqrt{2\pi} < b^2
    \end{cases}
    \\
\end{split}
\end{equation}
%
\begin{equation}
\begin{split}
    T_2 + |T_1|
    =& - \frac{2b}{\sqrt{2\pi}}\cdot E_1
        + \exp(-c) + (b^2+1) T_q
        + b(T_{q,1} - T_{q,2})
    \leq \exp(-c) + (b^2+b+1) T_q
    \\
    =& \exp(-c) + (b^2+b+1) \exp\Big(\frac{b^2}{2}-c\Big) \cdot \I\{c-\log\sqrt{2\pi} \geq b^2\}
        \\
        &\ + \frac{2b^3(b^2+b+1)}{(b^2 + c-\log\sqrt{2\pi})(b^2 - c+\log\sqrt{2\pi})} \cdot E_1
    \\
    \leq& (b+1)^2\exp\big(-\frac{c}{2}\big) \cdot \I\{c-\log\sqrt{2\pi} \geq b^2\} + \exp(-c) + \frac{2(b+1)}{1 - (\frac{c-\log\sqrt{2\pi}}{b^2})^2} E_1
    \\
    \lesssim& \begin{cases}
        (b+1)^2\exp(-\frac{c}{2}) - \Theta(b) E_1,
        & c-\log\sqrt{2\pi} \geq b^2
        \\ 
        \exp(-c) + \Theta(b) E_1,
            & c-\log\sqrt{2\pi} < b^2
    \end{cases}
    \\
    \lesssim& \begin{cases}
        (b+1)^2 \exp(-\frac{c}{2}), & c-\log\sqrt{2\pi} \geq b^2
        \\
        \Theta(b) E_1, & c-\log\sqrt{2\pi} < b^2
    \end{cases}
\end{split}
\end{equation}
% 
Hence 
\begin{equation}
\begin{split}
    &\sigma_{\min} \geq \frac{T_2 T_0 - |T_1|^2}{T_2 + |T_1|}
    \geq \begin{cases}
        \frac{\exp(b^2) - 1 - 2b\exp(\frac{b^2}{2})}{(b+1)^2} \exp\left(-\frac{3}{2}c\right),
        & c-\log\sqrt{2\pi} \geq b^2
        \\
        \Theta(b^3) E_1,
        & c-\log\sqrt{2\pi} < b^2
    \end{cases}
\end{split}
\end{equation}
%
\textcolor{orange}{// Problematic when $c \gg b^2$}
\begin{equation}
\begin{split}
    T_q \simeq& \exp\left(\frac{b^2}{2}-c\right) - O\left(\frac{b}{c}\right)\exp\left(-\frac{c}{b^2}\cdot \frac{c}{2}\right)
\end{split}    
\end{equation}

\textcolor{RoyalBlue}{// Lower bound even further}

\begin{equation}
\begin{split}
    T_2 - T_0
    = b^2 T_q + (R-b)^2 T_{*,1} + (R+b)^2 T_{*,2} + E
\end{split}
\end{equation}

When $T_2 > T_0$,
\begin{equation}
\begin{split}
    \sigma_{\min} \geq \frac{T_2 T_0 - |T_1|^2}{T_2 + |T_1|}
    = \frac{\sqrt{T_2 T_0} + |T_1|}{\sqrt{T_2 T_2} + |T_1|} \cdot  (\sqrt{T_2 T_0} - |T_1|)
    \geq \sqrt{\frac{T_0}{T_2}} (\sqrt{T_2 T_0} - |T_1|)
    = T_0 - \sqrt{\frac{T_0}{T_2}} \cdot |T_1|
    \\
\end{split}
\end{equation}
%
When $T_0 > T_2$,
\begin{equation}
\begin{split}
    \sigma_{\min} \geq \frac{\sqrt{T_2 T_0} + |T_1|}{\sqrt{T_2 T_2} + |T_1|} \cdot  (\sqrt{T_2 T_0} - |T_1|)
    \geq \sqrt{T_2 T_0} - |T_1|
    = T_0 - \sqrt{\frac{T_0}{T_2}} \cdot |T_1| 
\end{split}
\end{equation}

When $\frac{c-\log\sqrt{2\pi}}{b} \leq \frac{R}{2}$, $E_1 \geq E_2$,
\begin{equation}
\begin{split}
    \sigma_{\min} \geq T_0 - \sqrt{\frac{T_0}{T_2}} \cdot |T_1|
    \geq T_q - \frac{}{}
\end{split}
\end{equation}

When $\frac{c-\log\sqrt{2\pi}}{b} \in [-b, b]$,
\textcolor{midgray}{\textcolor{orange}{NOTE}: don't do this case-by-case: there're 5 cases}
\begin{equation}
\begin{split}
    T_0 \simeq& \left(\frac{b}{b^2 - c + \log\sqrt{2\pi}} +\frac{b}{b^2 + c - \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(c-\log\sqrt{2\pi})^2}{2b^2}\right)
        \\
        &\ + \left(\frac{b}{b(R+b) - c + \log\sqrt{2\pi}} + \frac{b}{b(R-b) - c + \log\sqrt{2\pi}}\right) \cdot \exp\left(-\frac{(\frac{c-\log\sqrt{2\pi}}{b}-R)^2}{2}\right)
\end{split}
\end{equation}

% \begin{equation}
% \begin{split}
%     \frac{T_0 - \frac{|T_1|}{T_2} |T_1|}{1 + \frac{|T_1|}{T_2}}
% \end{split}
% \end{equation}

% Substituting $T^{(0)}, T^{(1)}, T^{(2)}$ back to equation \ref{eq:nce_sigma_min_lb} gives:
% \begin{equation}
% \begin{split}
%     \sigma_{\min}(\nabla^2 L)
%     \geq& \frac{T_2 T_0 - T_1^2}{T_2 + |T_1|}
%     \\
%     =& \frac{}{}
% \end{split}
% \end{equation}

In particular, for $[b,c] \in \gA$, we have 
\begin{equation}
\begin{split}
    T^{(0)} =& \Theta(1/R) \exp\left(-\frac{c^2}{2b^2}\right)
        + \Theta(1/R) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
    \\
    T^{(1)} =& \Theta(1) \exp\left(-\frac{c^2}{2b^2}\right)
        + \Theta(1) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
    \\
    T^{(2)} =& \Theta(R) \exp\left(-\frac{c^2}{2b^2}\right)
        + \Theta(R) \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)
\end{split}
\end{equation}
where we omitted $-\log\sqrt{2\pi}$ in $c-\log\sqrt{2\pi}$ since $c \gg \log\sqrt{2\pi}$.

Let $E_{\max} := \left\{\exp\left(-\frac{c^2}{2b^2}\right),\ \exp\left(-\frac{(\frac{c}{b}-R)^2}{2}\right)\right\}$.
$E_{\max}$ can be written as $E_{\max} = \exp\left(-\frac{\kappa(b,c) \cdot R^2}{8}\right)$ where $\kappa(b,c) \in [\frac{3}{4}, \frac{5}{4}]$ is the constant defined in equation \ref{eq:grad_ring_0th}.

Substituting $T^{(0)}, T^{(1)}, T^{(2)}$ back to equation \ref{eq:nce_sigma_min_lb} gives:
\begin{equation}
\begin{split}
    \sigma_{\min}(\nabla^2 L) \geq \frac{T^{(2)} T^{(0)} - (T^{(1)})^2}{T^{(2)} + |T^{(1)}|}
    = \frac{\Theta(1) \cdot E_{\max}^2}{\Theta(R) \cdot E_{\max}}
    = \Theta(1/R) \cdot E_{\max}
    = \Theta(1/R) \exp\left(-\frac{\kappa(b,c) \cdot R^2}{8}\right)
\end{split}
\end{equation}
which completes the proof.


==> proofs/not_used/claim_3rd_dev_prev_attempts.tex <==

\textcolor{RoyalBlue}{Goal}:
\textcolor{gray}{
We want to show that there exists some $C = \poly(\|\param_* - \param_q\|, \kappa_*)$, such that $\forall \vv$,
\begin{equation}
\begin{split}
    2\nabla_{\param_*}^3 L (\vv, \vv, \vv)
    =& \int_x \frac{p_*q}{p_*+q} \frac{q-p_*}{p_*+q} (\vv^\top T(x))^3
    = \int_x \frac{p_*q}{p_*+q} (\vv^\top T(x))^2 \cdot \frac{q-p_*}{p_*+q} (\vv^\top T(x))
    \\
    \leq& C \max_{\vu} \int_x \frac{p_*q}{p_*+q} (\vu^\top T(x))^2
\end{split}
\end{equation}
}

\textcolor{RoyalBlue}{Subgaussian diameter?} \textcolor{gray}{If $T(x)$ is bounded, i.e. $\|T(x)\| \leq c_T$ for some $c_T$, then it trivially holds that
\begin{equation}
\begin{split}
    2\nabla_{\param_*}^3 L (\vv, \vv, \vv)
    \leq c_T \int_x \frac{p_*q}{p_*+q} \left|\vv^\top T(x)\right|^2
\end{split}
\end{equation}
It is hence plausible that even though $T(x)$ is not bounded, it may have a ``subgaussian diameter" (e.g. \href{https://arxiv.org/abs/1309.1007}{Kontorovich 13}) that serves the same purpose.
}


\textcolor{RoyalBlue}{Fact}
\textcolor{gray}{(\href{https://web.math.princeton.edu/~rvan/APC550}{page 55}):
If $X$ is $\sigma^2$-subgaussian, then $\E[X^{2q}] \leq (4\sigma^2)^{q}q!$ for all $q \in \N$.
}


\textcolor{RoyalBlue}{\textit{Side note}}: \textcolor{gray}{Can we show: $\forall p, q$, 
$\int_{x} \frac{pq}{p+q}(\vv^\top T(x))^2
\leq \int_x \frac{p}{2} (\vv^\top T(x))^2
= \frac{1}{2} \E_{P}[(\vv^\top T(x))^2]
$.
}


==> proofs/not_used/ence_sigma_bdd_option1.tex <==
\textcolor{RoyalBlue}{\textbf{Option 1}}: we prove this under the assumption that $\gS_+(\vv), \gS_-(\vv) \subset \{x: \bar\delta^\top T(x) < 0\}$.

Let $\gS(\vv)$ denote the set s.t. $\int_{x\in \gS(\vv)} p_{\frac{\theta_*+\theta_q}{2}}(x) (\vv^\top T(x))^2 = \frac{1}{2}\int_x p_{\frac{\theta_*+\theta_q}{2}}(x) (\vv^\top T(x))^2$,
and \textcolor{peach}{assume $\gS(\vv) \subset \{x: \bar\delta^\top T(x) > 0\}$}, for all unit vector $\vv$;
the other case, i.e. $\gS(\vv) \supset \{x: \bar\delta^\top T(x) > 0\}$, is symmetric.
\textcolor{orange}{We will show that $\gS_+(\vv), \gS_-(\vv) \subset \{x: \bar\delta^\top T(x) > 0\}$ if $\|\bar\delta\| \ll \|\param(\frac{\theta_*+\theta_q}{2})\|$.}
(\textcolor{red}{todo})

Let $\vv = \ve_{-1}$, i.e. $\vv^\top T(x) = -1$.
Then $\gS_+(\vv) \subset \{x: \bar\delta^\top T(x) < 0\}$ means:
\begin{equation}
\begin{split}
    \int_{x: \bar\theta^\top \tilde{T}(x) > -\bar\alpha} \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) + \bar\theta^\top \tilde{T}(x)\right)
    % \geq \frac{1}{2} \int_x \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) + \bar\theta^\top \tilde{T}(x)\right)
    \geq \frac{1}{2} Z(\bar\theta + \frac{\theta_q+\theta_*}{2})
\end{split}
\end{equation}
Hence the ratio in partition function is upper bounded by:
\begin{equation}
\begin{split}
    \frac{Z(-\bar\theta + \frac{\theta_q+\theta_*}{2})}
            {Z(\bar\theta + \frac{\theta_q+\theta_*}{2})}
    =&\ \frac{\int_x \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) - \bar\theta^\top \tilde{T}(x)\right)}
        {\int_x \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) + \bar\theta^\top \tilde{T}(x)\right)}
    \\
    \leq&\ 2\frac{\int_{x:\bar\theta^\top \tilde{T}(x)>-\bar\alpha}  \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) - \bar\theta^\top \tilde{T}(x)\right)}
        {\int_{x:\bar\theta^\top \tilde{T}(x)>-\bar\alpha}  \exp\left(\frac{(\theta_q+\theta_*)^\top}{2} \tilde{T}(x) + \bar\theta^\top \tilde{T}(x)\right)}
    \leq 2\exp\left(-\bar\alpha\right)
\end{split}
\end{equation}
Substituting this back to equation \ref{eq:kappa_tilde_bound_part1} gives 
\begin{equation}\label{eq:kappa_tilde_bound_part2}
\begin{split}
    \kappa(\mH(\tilde\delta))
    \leq& \kappa(\mH_*) \cdot 2\exp(2|\bar\alpha|)
        \cdot \frac{\lambda_{\max}^2}{\lambda_{\min}^2}
        \cdot \left(1 + 2\exp(-\bar\alpha) \right)
    \\
    \leq& 4\exp\left(4|\bar\alpha|\right) \cdot \frac{\lambda_{\max}^2}{\lambda_{\min}^2} \cdot \kappa(\mH_*)
    \leq 4\exp\left(4\right) \cdot \frac{\lambda_{\max}^2}{\lambda_{\min}^2} \cdot \kappa(\mH_*)
    = O\left(\frac{\lambda_{\max}^2}{\lambda_{\min}^2}\right) \cdot \kappa(\mH_*)
\end{split}
\end{equation}

==> proofs/not_used/lem_ngd_loss_two_cases.tex <==
We will prove two cases separately, one for $\param$ that is at some distance away from $\param_*$, and one for $\param$ close to $\param_*$.
When $\delta > 1$, the first case is sufficient for the proof. \Bnote{double check}
When $\delta< 1$, we choose $\gamma$ such that the sets of parameters corresponding to the two cases overlap, hence the two cases cover all choices of $\param$ and the proof is done.

\textbf{Case 1: faraway $\param$}: Intuitively, by convexity, $L(\param_* + \drop\frac{g_t}{\|g_t\|}) \leq L(\param)$ is easily satisfied when $\|\param - \param_*\|_2 \gg \drop$.
Formally, we want to find a threshold $r \geq \drop$ s.t. the following lemma holds:
\begin{lemma}
\label{lem:ngd_case1}
    There exists $r \geq \drop$,
    such that $\forall \param_1 \in \gB(\param_*, \drop)$, $\param_2 \not\in \gB(\param_*, r)$, $L(\param_1) \leq L(\param_2)$.
\end{lemma}
\begin{proof}
    Let $\maxloss := \max_{\param \in \gB(\param_*, \drop)} L(\param)$,
    then $r$ can be chosen as $r := \arg\max_{\param: L(\param)\leq\maxloss}\|\param - \param_*\|_2$.
    In words, we consider the level set specified by the max function value within the ball $\gB(\param_*, \drop)$, and let $r$ be the max distance between points in the level set to $\param_*$.
\end{proof}
Let $\sigma_{\max}^*, \sigma_{\min}^*$ denote the maximum and minimum singular value of $\mH_*$.
For $\drop \ll 1$, $\frac{r}{\drop}$ is the condition number of $\mH_*$, since for any unit vector $\vv$ and constant $c \in O\left(\frac{1}{\TxBdd \kappa_*}\right)$,
\begin{equation}
\begin{split}
    L(\param_* + c\vv) - L(\param_*)
    =& \frac{c^2}{2}\vv^\top \mH_*\vv + O(\|\nabla^3_{\param_*} L\|_{\max}c^3)
    \in \left[\frac{\sigma_{\min}^*c^2}{2}, \frac{\sigma_{\max}^*c^2}{2}\right] + O(\TxBdd \kappa_*c^3)
\end{split}
\end{equation}
The $O(\TxBdd \kappa_*c^3)$ term is dominated by $\sigma_{\min}^*$ and $\sigma_{\max}^*$ by the choice of $c$ and Claim \ref{clm:3rd_dev}.

\textbf{Case 2: near-optimal $\param$}:
For $\delta \in O\left(\frac{1}{\TxBdd\kappa_*}\right)$,
consider $\param$ s.t. $\delta \leq \|\param - \param_*\|_2 \in O\left(\frac{1}{\TxBdd\kappa_*}\right)$.
The losses at $\param_* + \drop\frac{g_t}{\|g_t\|}$ and $\param_t$ are:
\begin{equation}
\begin{split}
    &L\left(\param_* + \drop\frac{g_t}{\|g_t\|}\right)
    = L(\param_*) + \frac{\drop^2}{2\|g_t\|^2}g_t^\top \mH_* g_t + O(\TxBdd \kappa_*\sigma_{\min}^*\|\drop\|^3)
    \\
    % =& L(\param_*) + \frac{c^2}{2\|g_t\|^2}(\param-\param_*)^\top \mH_*^\top \mH_* \mH_* (\param-\param_*) + O(c^3)
    % \\
    % =& L(\param_*) + \frac{\drop^2}{2\|g_t\|^2}(\param-\param_*)^\top \mH_*^3 (\param-\param_*) + O(\|\nabla^3_{\param_*} L\|_{\max}\drop^3)
    \\
    &L(\param) = L(\param_*) + \frac{1}{2}(\param-\param_*)^\top \mH_* (\param-\param_*) + O(\TxBdd \kappa_*\|\param-\param_*\|^3)
\end{split}
\end{equation}

% \TODO{update the $\drop^3$ term to depend on $\mH_*$; this is where we need info about NCE:
% \footnote{We need the property about NCE that even though the loss/gradient/Hessian (and higher order derivatives) are exponentially small, they share the same exponential order which can cancel out.
% (side note: we need to update TRE notes as well for the same issue)}
% make this clear somewhere.
% W/o this property, in order for the second term to dominate $\drop^3$, we must have $\drop \leq \sigma_{\min}^*$, which could itself be exponentially small}


In order to have $L\left(\param_* + \drop\frac{g_t}{\|g_t\|}\right) \leq L(\param)$, we need 
\begin{equation}
\begin{split}
    & \frac{\drop^2}{\|g_t\|^2}g_t^\top \mH_* g_t \leq (\param-\param_*)^\top \mH_* (\param-\param_*),\ \forall \param \text{ s.t. } \|\param -\param_*\|_2 \geq \delta
    \\
    \Rightarrow& \drop^2 \leq \frac{(\param-\param_*)^\top \mH_* (\param-\param_*)}{\frac{g_t^\top}{\|g_t\|}\mH_*\frac{g_t}{\|g_t\|}},\ \forall \param \text{ s.t. } \|\param -\param_*\|_2 \geq \delta 
    % \\
    \Rightarrow \drop \leq \sqrt{\frac{\sigma_{\min}^*}{\sigma_{\max}^*}} \delta
    = \frac{\delta}{\sqrt{\kappa_*}}
    \\
\end{split}
\end{equation}
Therefore, choose constant $c \in \Theta\left(\frac{1}{\TxBdd \kappa_*}\right)$ and set $\drop = \frac{c\delta}{\sqrt{\kappa_*}} = \Theta$, ensures the sets of $\param$ covered by case 1 and 2 overlap, i.e. $r = \frac{r}{\drop} \cdot \drop = \kappa_* \cdot O\left(\frac{1}{\poly(\kappa_*)}\right) \delta
= O\left(\frac{1}{\poly(\kappa_*)}\right) \delta \ll 1$.


==> proofs/not_used/old_nce_sigmas.tex <==
\subsection{Singular values around \texorpdfstring{$\param_*$}{optimal parameter}}

We would like to show that when $\|\param - \param_*\|_2 \leq \frac{1}{\logLipsZ}$, the Hessian at $\param$ has singular values multiplicatively close to those at $\param_*$.

\textcolor{midgray}{// $P_*, Q$ being close may not help, since we only require $\|\theta_* - \theta_q\| = O\left(\frac{1}{\lambda_{\max}}\right)$, rather than the small value as required by Taylor expansion.}

Let $\param = \param_* + \delta$, and write $\delta = [\bar\theta, \bar\alpha]$.
\begin{equation}\label{eq:nce_sigma_ub}
\begin{split}
    &\vv^\top \nabla^2 L(\param) \vv
    = \int_{\delta^\top T(x) < 0} (p_* + q) \frac{pq}{(p+q)^2} (\vv^\top T(x))^2 dx
        + \int_{\delta^\top T(x) > 0} (p_* + q) \frac{pq}{(p+q)^2} (\vv^\top T(x))^2 dx
    \\
    \overset{(i)}{\leq}& \frac{Z(\frac{\theta_*+\theta_q}{2})}{\sqrt{Z(\theta_*)Z(\theta_q)}} \lambda_{\max}
        \cdot \left(2\exp\left(1+\frac{1}{\logLipsZ}\right) + \exp\left(\frac{3}{2}+\frac{1}{\logLipsZ}\right)\right)
    \\ 
    % \leq \int_x \frac{p_* + q}{p + q} \min\{p, q\} (\vv^\top T(x))^2 dx
    % \\
    % =& \int_x \frac{p_* + q}{p_* \exp\left(\delta^\top T(x)\right) + q} \min\{p, q\}  (\vv^\top T(x))^2 dx
    % \\
    % \leq& \int_{\delta^\top T(x) < 0} \frac{p_* + q}{p_* \exp\left(\delta^\top T(x)\right) + q} \min\{p_*, q\}  (\vv^\top T(x))^2 dx
    %     + \int_{\delta^\top T(x) > 0} \min\{p, q\}  (\vv^\top T(x))^2 dx
    % \\
\end{split}
\end{equation}
where step $(i)$ uses calculations in equation \ref{eq:nce_sigma_ub_t1} and \ref{eq:nce_sigma_ub_t2}.

\input{proofs/nce_sigmas_ub}

\textcolor{gray}{\textcolor{orange}{TODO}: lower bound}



==> proofs/prop_1dG_loss.tex <==
\subsection{Proof of Proposition \ref{prop:opt_loss} (range of the NCE loss)}

\TODO{add proof}

==> proofs/prop_loss_to_dist.tex <==
\subsection{Proof of Proposition \ref{prop:loss_to_dist} (excess loss to parameter distance)}

\TODO{add proof}

==> proofs/thm_expNCE.tex <==
\subsection{Proof of Theorem \ref{thm:nce_exp_ngd} (\ENCE\ convergence)}

% \begin{theorem}[Theorem \ref{thm:nce_exp_ngd} restated]
% \label{thm:nce_exp_ngd_restate}
%     Under assumption \ref{assump:param_norm_bdd} - \ref{assump:Tx_2nd3rd},
%     let $P_*, Q$ be exponential family distributions with parameters $\param_*, \param_q$.
%     For any given $\delta > 0$ and parameter initialization $\param_0$,
%     performing NGD on the \ENCE objective finds a $\param$ such that $\|\param - \param_*\|_2 \leq \delta$ within $O\left(\frac{\|\param_0 - \param_*\|^2}{\delta^2}\paramDeriv\right)$, where $\paramDeriv$ is the constant in assumption \ref{assump:Tx_bdd}.
% \end{theorem}
% \begin{proof}
We have seen in the proof of Lemma \ref{lem:nce_exp_kappa} that the \ENCE\ loss is convex for the exponential family.
The only thing left to do is show that \ENCE\ also satisfies part (ii) of Assumption \ref{assump:hessian_neighbor}:
\begin{lemma}
\label{clm:sigma_bdd_exp}
Under assumption \ref{assump:log_lips} with constant $\logLipsZ$,
for any unit vector $\vu$ and constant $c \in [0, \frac{1}{\logLipsZ}]$,
the maximum and minimum singular values of $\mH(\param_* + c\vu)$ satisfy assumption \ref{assump:hessian_neighbor} with constants
$\cSigmaMaxNB = 2\exp(1) \cdot \frac{\lambda_{\max}}{\lambda_{\min}}$,
$\cSigmaMinNB = \frac{1}{2\exp(1)} \cdot \frac{\lambda_{\min}}{\lambda_{\max}}$.
\end{lemma}
The proof of this is included in Appendix~\ref{appendix:ence_sigma_bdd}. With Assumption \ref{assump:hessian_neighbor} established, Theorem \ref{thm:ngd} can be applied and the proof is complete.
% \end{proof}


==> proofs/thm_ngd.tex <==
% \subsection{Proof of Theorem \ref{thm:ngd} (NGD convergence rate)}
% \label{subsec:proof_thm_ngd}

% \begin{theorem}[Theorem \ref{thm:ngd} restated]
%     \label{thm:ngd_restated}
%     Let $L$ be any loss function that is convex in the exponential family parameter and satisfies Assumptions  \ref{assump:hessian_neighbor} and \ref{assump:param_norm_bdd} - \ref{assump:bdd_3rd_dev}. Furthermore, let $P_*,Q$ be exponential family distributions with parameters $\param_*, \param_q$ and 
%     let $\kappa_*$ be the condition number of the Hessian at $P=P_*$.
%     % \anote{with what step size?}
%     Then, for any $0 < \delta \leq \frac{1}{\logLipsZ}$ and parameter initialization $\param_0$,
%     let the step size be $\eta \leq \sqrt{\frac{\cSigmaMinNB}{\cSigmaMaxNB\kappa_*}} \delta$,
%     performing NGD on the population objective $L$ guarantees that after $T \leq \frac{\cSigmaMaxNB\kappa_*}{\cSigmaMinNB} \cdot \frac{\|\param_0 - \param_*\|^2}{\delta^2}$ steps,
%     there exists an iterate $t \leq T$ such that 
%     $\|\param_t - \param_*\|_2 \leq \delta$.
%     % finds an estimate $\param$ such that $\|\param - \param_*\|_2 \leq \delta$ within $T = \frac{\cSigmaMaxNB\kappa_*}{\cSigmaMinNB} \cdot \frac{\|\param_0 - \param_*\|^2}{\delta^2}$ steps,
% \end{theorem}
% 
\begin{proof}
Denote $g_t := \nabla L(\param_t)$ and $R := \|\param_* - \param_q\|_2$ for notation convenience.
Recall that the NGD update with step size $\eta$ is $\param_{t+1} = \param_{t} - \eta \cdot \frac{g_t}{\|g_t\|_2}$.
% For a convexity function $f$ minimized at $\param_*$
% and exponential families with parameter $\param$, i.e. $p_{\param}(x) = \exp(\param^\top T(x))$,
% \footnote{Recall that the log partition function is included in $\param$, with $-1$ as its corresponding coordinate in $T(x)$.}
% 
% \input{ngd/deprecated/old_calc_ngd_outline.tex}
% 
Then, $\|\param_{t} - \param_*\|^2$ can be rewritten as:
\begin{equation}
\begin{split}
    \|\param_{t+1} - \param_*\|^2
    % =& \|\param_t - \param_*\|^2 - 2\eta\frac{g_t^\top}{\|g_t\|}(\param_t - \param_*) + \eta^2
    % \\
    % = \|\param_t - \param_*\|^2 + 2\eta\frac{g_t^\top}{\|g_t\|}\left(\param_* + \drop\frac{g_t}{\|g_t\|} - \param_t - \drop\frac{g_t}{\|g_t\|}\right) + \eta^2
    % \\
    =& \|\param_t - \param_*\|^2 - 2\drop\eta + \eta^2
        + 2\eta\frac{g_t^\top}{\|g_t\|}\left(\param_* + \drop\frac{g_t}{\|g_t\|} - \param_t\right)
\end{split}
\end{equation}
If we set $\drop$ s.t. the last term is smaller than 0 for all $\param$ that are not within distance $\delta$ to $\param_*$, setting $\eta = \drop$ gives:
\begin{equation}
\begin{split}
    \|\param_{t+1} - \param_*\|^2
    \leq \|\param_t - \param_*\|^2 - 2\drop\eta + \eta^2
    = \|\param_t - \param_*\|^2 - \drop^2
\end{split}
\end{equation}
Hence the number of steps required to find a $\param$ s.t. $\|\param- \param_*\|_2 \leq \delta$ is at most $T \leq \frac{\|\param_0 - \param_*\|^2}{\drop^2}$.

By Lemma \ref{lem:ngd_decrease_c}, setting $\drop = \sqrt{\frac{\cSigmaMinNB}{\cSigmaMaxNB\kappa_*}} \delta$ ensures 
% $\frac{g_t^\top}{\|g_t\|}\left(\param_* + \drop\frac{g_t}{\|g_t\|} - \param_t\right) \leq 0$
$L\big(\param_* + \drop\frac{g_t}{\|g_t\|}\big) \leq L(\param_t)$
for any $\param_t$ that is at least $\delta$ away from $\param_*$.
% Lemma \ref{lem:ngd_decrease_c} shows that such choice of $\drop$ guarantees $L\left(\param_* + \drop\frac{g_t}{\|g_t\|}\right) \leq L(\param_t)$, and
It then follows from the convexity of $L$ that
\begin{equation}
\begin{split}
    g_t^\top\left(\param_* + \drop\frac{g_t}{\|g_t\|} - \param_t\right)
    \leq L\left(\param_* + \drop\frac{g_t}{\|g_t\|}\right) - L(\param_t)
    \leq 0.
\end{split}
\end{equation}
Substituting this choice of $\drop$ back to the bound for $T$ gives $T \leq \frac{\cSigmaMaxNB\kappa_*}{\cSigmaMinNB} \cdot \frac{\|\param_0 - \param_*\|^2}{\delta^2}$
\end{proof}
